Who is More Bayesian: Humans or ChatGPT?

We compare the performance of human and artificially intelligent (AI) decision makers in simple binary classification tasks where the optimal decision rule is given by Bayes Rule. We reanalyze choices of human subjects gathered from laboratory experiments conducted by El-Gamal and Grether and Holt and Smith. We confirm that while overall, Bayes Rule represents the single best model for predicting human choices, subjects are heterogeneous and a significant share of them make suboptimal choices that reflect judgement biases described by Kahneman and Tversky that include the ``representativeness heuristic'' (excessive weight on the evidence from the sample relative to the prior) and ``conservatism'' (excessive weight on the prior relative to the sample). We compare the performance of AI subjects gathered from recent versions of large language models (LLMs) including several versions of ChatGPT. These general-purpose generative AI chatbots are not specifically trained to do well in narrow decision making tasks, but are trained instead as ``language predictors'' using a large corpus of textual data from the web. We show that ChatGPT is also subject to biases that result in suboptimal decisions. However we document a rapid evolution in the performance of ChatGPT from sub-human performance for early versions (ChatGPT 3.5) to superhuman and nearly perfect Bayesian classifications in the latest versions (ChatGPT 4o).

==> 2human_binary_classifications.tex <==
\label{section:wisconsin}

In this section we reanalyze experimental data on the decisions of human subjects
gathered from two separate experiments: 1) 257 student subjects from
four different universities in California reported in \citet{EGG1995}, and 2) 
79 student subjects at the University of Wisconsin reported in \citet{EGG1999}.
Both of these experiments involved simple binary classifications: subjects were shown a random sample
of draws from one of two bingo cages with known probabilities of being selected and  asked to choose the cage
that they believed was more likely to have been used to generate the observed sample.
We start by describing the experiments and the statistical decision theory framework
we use to evaluate the optimality of subjects' decisions.
We also introduce the ``structural logit'' model that forms the basis of our empirical reanalysis of
these data, and discuss the identification of ``revealed subjective posterior beliefs.'' These
beliefs were not directly reported by subjects in the experiment, but instead must be inferred from the binary sequences of
classification decisions made by the subjects. We defer to section 4 a separate reanalysis of
data gathered by \citet{HS2009} that does directly elicit subjects' subjective posterior beliefs.  

\subsection{Reanalysis of California Experiments}

We refer to the set of experiments run in California as the ``California design.'' They involved
two bingo cages, A and B, containing 6 balls in each marked with the letters N or G and a ``prior cage''
with 6 balls labelled  with numbers 1 to 6.  Each trial of the experiment began with a random draw from
the prior cage.  Subjects were informed that if the selected ball was numbered from 1 to $m$ (where $m \in \{2,3,4\}$)
a second set of balls would be drawn from cage A, otherwise the balls would be drawn from cage B.
The second set of draws from the selected cage (A or B) involved 6 draws at random and with replacement.
Let $n$ denote the number of balls out of the
6 in the random sample from  the selected cage that were marked N. Clearly, $n$ is a sufficient statistic
for the outcome of the six draws with replacement and has a binomial distribution with parameters $6$ and
$p$ where $p$ is the fraction of balls marked N in the chosen urn.
Cage A contained 4 N balls and 2 G balls, so the probability
of randomly sampling an N ball was $p_A=2/3$. Cage B contained 3 N balls and 3 G balls, so the
probability of drawing an N ball was $p_B=1/2$. 

The information provided to the subjects in each trial was $(\pi,n)$. The prior $\pi$
was actually communicated via a public announcement to the subjects of the integer $m$ that determined when cage A was drawn, so there were three
possible prior probabilities $\pi \in \{1/3,1/2,2/3\}$. Of course subjects were only told $m$ (which implies $\pi$)
but not the actual outcome of the draw from the prior cage. Based on this outcome, either cage A or B was selected
for the drawing of a random sample of 6 balls. The cages were placed behind an opaque screen so subjects
were unable to see the draw from the prior cage or which cage, A or B, had actually been selected for the second drawing. A student monitor was paid
to stand behind the opaque screen and verify that the announced rules for each trial were being followed and the outcomes
$(\pi,n)$ were truthfully reported thereby
resulting in a credible ``objective prior'' and likelihood for each observed trial outcome $(\pi,n)$.

\subsection{Bayes Rule, Decision Rules, and Statistical Loss Functions}

The conditional probability $\Pi(A|\pi,n)$ that cage A was used to draw the sample given the reported information
on any particular trial, $(\pi,n)$, is an objective posterior probability given by  Bayes Rule
\begin{equation}
    \Pi(A|\pi,n) =  {\pi f(n|A) \over \pi f(n|A) + (1-\pi) f(n|B)},
\label{eq:bayes_rule}
\end{equation}
where $f(n|A)={6 \choose n} p_A^n (1-p_A)^{6-n}$ and $f(n|B) = {6 \choose n}p_B^n (1-p_B)^{6-n}$.

\begin{definition}{\bf Decision Rule}
A decision rule is a conditional probability $P(A|\pi,n)$ of selecting cage A
as a function of the information $(\pi,n)$. 
\end{definition}

When $P(A|\pi,n)$ is a probability, i.e. $0 < P(A|\pi,n)< 1$, it is referred to as a {\it mixed strategy\/}
otherwise it is called a {\it pure strategy.\/} We allow for the extra flexibility of mixed strategies since the choices
of virtually all experimental subjects will be best approximated via a {\it conditional choice probability\/} (CCP) $P(A|\pi,n)$
rather than a deterministic function of $(\pi,n)$, and hence we can identify the estimated CCP  as the mixed
strategy used by subjects in the experiment.

Some of the subjects in the experiment were incentivized by being
offered a \$10 bonus if they selected the correct cage used to draw the sample in a randomly selected trial in the experiment. 
However this payment was made {\it after\/} all trials were completed. Beyond an initial description of the bingo cage setup
and a single demonstration of how it works at the start of the experiment, {\it none of the subjects received any feedback on whether they
had selected the correct cage after each trial in the experiment.\/} This was evidently an intentional feature of the experimental
design, to reduce the possibilities of non-stationarity in subjects' decision rules during the experiment due to
``learning effects'' that are enhanced via real-time feedback. 

Even though some of the subjects were not incentivized via a bonus payment for selecting the correct cage in a randomly
selected trial, the main difference between the incentivized and non-incentivized subjects was that the estimated error 
probability $\varepsilon$ (i.e the probability a subject would randomly guess cage A or B) was significantly lower in the incentivized
experiments. But overall, it seems reasonable to presume that both incentivized and non-incentivized subjects were trying
to maximize the probability of selecting the correct cage, i.e. the actual cage used to draw the sample of 6 balls. 
In other words, it is reasonable to presume that subjects in the experiment would prefer to use
an {\it optimal decision rule\/} if it was not too difficult for them to calculate, or some approximation to it
otherwise.

\begin{definition}{\bf Optimal decision rule}
An optimal decision rule $P^*(A|\pi,n)$ is one that maximizes the probability of selecting the actual cage 
used to draw the sample.
\end{definition}

The following Lemma justifies our interest in Bayes Rule as a ``normative rule'' for subject behavior. We don't focus
on Bayes Rule because many statisticians believe it a fundamental implication of probability
theory and thus a basic principle of logical behavior or an axiom of how people ``ought to learn''. Instead, greedy subjects (i.e. those who 
are trying to maximize their payoff from the experiment) should act ``as if'' they are following Bayes Rule simply
because they are selfish maximizers who would like to adopt a decision rule that maximizes their payoff from participating in the experiment.

\begin{lemma}
\label{lemma:bayes_optimality}
The optimal decision rule in the El-Gamal and Grether binary classification experiment is the pure strategy
defined in terms of  Bayes Rule
\begin{equation}
    P^*(A|\pi,n) = \left\{\begin{array}{ll}
            1 & \mbox{if} \;\; \Pi(A|\pi,n) \ge 1/2 \cr
            0 & \mbox{otherwise}.
\label{eq:optpure}
\end{array}
\right. 
\end{equation}
\end{lemma}
                     
It is convenient to define two binary random variables, $\tilde W_P$ and $\tilde L_P$, implied by decision rule $P$ by
$\tilde W_P=1$ if the subject selects the correct cage from which the sample was drawn, and 0 otherwise. Thus, $\tilde W_P$
is an indicator for a ``win'' i.e. a correct prediction or classification. $\tilde L_P$ is the indicator for a loss,
i.e. an incorrect prediction. It follows that with probability 1 we have $1=\tilde W_P+\tilde L_P$, and so we can define
an optimal decision rule as one that maximizes the probability of a win or conversely one that minimizes the probability
of a loss. Following the standard terminology from the literature on statistical decision theory, we define

\begin{definition}{\bf Loss Function} The loss function is the conditional  probability of a loss,
\begin{equation}
    L_P(\pi,n) = E\{\tilde L_P|\pi,n\} = P(A|\pi,n)[1-\Pi(A|\pi,n)]+[1-P(A|\pi,n)]\Pi(A|\pi,n).
\label{eq:lossdef}
\end{equation}
\end{definition}
It is straightforward to see that an optimal decision rule $P$ must minimize
expected loss, and then using equation (\ref{eq:lossdef}) it follows immediately that the optimal
decision rule is the pure strategy (\ref{eq:optpure}) defined in terms of Bayes Rule.

Note that the loss function $L_P(\pi,n)$ conditions on specific experimental realizations, $(\pi,n)$. We can define
a {\it ex ante\/} or unconditional expected loss by first taking expectations over the unconditional distribution
of the number of N balls $n$
\begin{equation}
    L_P(\pi) = E\{\tilde L_P|\pi\} = \sum_{n=0}^6 L_P(\pi,n)[f(n|A)\pi+f(n|B)(1-\pi)],
\end{equation}
and then given a ``prior distribution over priors'' $F(\pi)$ we can calculate an overall {\it ex ante \/} expected
loss that a subject using decision rule $P$ will incur at the start of the experiment
\begin{equation}
    L_P = E\{\tilde L_P\} = \int_0^1 E\{\tilde L_P|\pi\}dF(\pi).
\end{equation}
We will use $L_P$ as a single summary statistic for the degree of suboptimality of a decision rule $P$ 
using our econometric estimates of $P$ from our structural logit model of subject choice behavior discussed below.
We use a uniform distribution over priors $F(\pi)$, although other distributions (such as the empirical distribution
of values of $\pi$ used in the actual experiments) could be used as well. Overall conclusions about
subject optimality do not depend a particular choice of $F$ and we also plot the entire conditional expected loss
$L_P(\pi)$ function for more insight into where the biggest  decision losses occur.

\subsection{Structural Logit Model of Subject Decision Making}

As we noted in the introduction, \citet{EGG1995} introduced an innovative model of subject decision making based
on the hypothesis that subjects employ {\it cutoff rules\/} to decide whether, given the outcome of a given trial
in the experiment $(\pi,n)$, the sample was drawn from cage A or cage B. Since cage A has a higher fraction of
N balls $p_A=2/3$, a plausible cutoff rule involves choosing cage A if $n > c_\pi$ where $c_\pi$ is a prior-specific
threshold.  In the California design there were three possible priors, $\pi \in \{1/3,1/2,2/3\}$ so there are  512
possible cutoff rules $(c_{1/3},c_{1/2},c_{2/3})$ that could be used.  For example, Bayes Rule corresponds to the
cutoff rule $c=(c_{1/3},c_{1/2},c_{2/3})=(4,3,2)$. However the cutoff rule model is {\it statistically degenerate\/}
i.e. for most subjects observed over $T$ successive trials, none of the cutoff rules will be able to perfectly predict the subject's choices.
To deal with this and avoid a ``zero likelihood problem'' \citet{EGG1995} introduced an additional error rate parameter
$\varepsilon \in (0,1)$ which has the interpretation as the probability that the subject guesses one of the cages
at random rather than use the cutoff rule. This results in a non-degenerate choice probability (decision rule) given by
\begin{equation}
   P(A|\pi,n) = \left\{\begin{array}{ll} 1-\frac{\varepsilon}{2} & \mbox{if}\;\; n > c_\pi \cr
                    \frac{\varepsilon}{2} & \mbox{otherwise}
\end{array}
\right.
\label{eq:eggprob}
\end{equation}
Using the choice probability $P(A|\pi,n)$ in equation (\ref{eq:eggprob}), \citet{EGG1995}
were able to write a likelihood function of the sequence of choices made by each subject in the
$T$ experimental trials in the experiment,  and estimate the four unknown
parameters of their model, $\theta=(c_{1/3},c_{1/2},c_{2/3},\varepsilon)$ by maximum likelihood. 
Though the model is innovative and interpretable,
it has several drawbacks that lead us to abandon it in favor of the structural logit model we introduce
below.  First the cutoff rule parameters are restricted to a finite grid 
of 8 possible integer values between -1 and 6, but this restricts the ability of the model to fit the
data and requires the use of non-standard asymptotics since the $c$ cutoff parameters will converge faster
than $\sqrt S$ (where $S$ is the total number of subjects in the experiment) to a non-normal limiting distribution.
Second, the nature of subject ``errors'' implied by their model is not entirely plausible: the probability
that a subject randomly guesses, $\varepsilon$, does not depend on the strength of the evidence the subject observes. 
For example, for values $(\pi,n)$ where the Bayesian posterior probability is close to 0 or 1, the subject should
realize this  and be clear that either cage A or B should be chosen. Random guesses should only be likely in the
more ambiguous cases where the Bayesian posterior is close to 1/2. 

A final shortcoming is that the
estimated cutoff rule parameters are not ``structural'' i.e. they are not invariant to an alteration of the experimental design. 
In the next section we describe an alternative experimental design that \citet{EGG1999} used for the experiments
at the University of Wisconsin where 7 balls were drawn from cages containing 10 balls each and different values
of $p_A=.4$ and $p_B=.6$ were used. Now, the cutoff rules estimated from the California experiments are no longer relevant:
subjects should be {\it less likely\/} to choose cage A when $n$ is larger. So the cutoff rule is reversed (i.e. cage A should
be chosen when $n$ is smaller than a given threshold $c_\pi$) and different
cutoffs are required to implement Bayes Rule in this situation. A good structural model should depend on parameters
that are {\it policy invariant\/} and do not change when the experiment (``policy'') is changed.

We now introduce a {\it structural logit model\/} that avoids these limitations and which includes the optimal
Bayesian decision rule $P^*(A|\pi,n)$ as a special case.
Similar to the El-Gamal and Grether model, the structural
logit model depends only 4 unknown parameters $\theta=(\beta_0,\beta_1,\beta_3,\sigma)$ where the first three parameters
are allowed to take any real value and determine the subject's subjective posterior beliefs. The last parameter $\sigma$ is
restricted to be positive and determines the level of idiosyncratic ``noise'' affecting the subject's final choice. 

Consider first the subject's subjective posterior beliefs which we denote by $\Pi_s(A|\pi,n)$. We presume that subjects
are able to transform the observed information $(\pi,n)$ into the pair $(\mbox{LPR}(\pi),\mbox{LLR}(n))$ where $\mbox{LPR}(\pi)$ is the log
posterior odds ratio and $\mbox{LLR}(n)$ is the log-likelihood ratio given by
\begin{eqnarray} 
     \mbox{LPR}(\pi) & = & \log(\pi/(1-\pi)) \nonumber \\
     \mbox{LLR}(n) & = &  \log(f(n|A)/f(n|B)).
\end{eqnarray}
After these transformations of the ``inputs'' $(\pi,n)$ we can write the subjective posterior in terms of the belief
parameters $\beta$ as
\begin{equation}
       \Pi_s(A|\pi,n,\beta) = {1 \over 1 + \exp\{\beta_0+\beta_1 \mbox{LLR}(n) + \beta_2 \mbox{LPR}(\pi)\} }.
\label{eq:subjectiveposterior}
\end{equation}
Notice that the true Bayesian posterior $\Pi(A|\pi,n)$ given in equation (\ref{eq:bayes_rule}) emerges as a special
case of the subjective posterior belief specification $\Pi_s(A|\pi,n,\beta)$ when $\beta=(0,-1,-1)$.  For other values
of $\beta$ the subjective posterior can capture a number of well known biases observed in past studies, including
an outright bias for cage A or B ($\beta_0 \ne 0$) as well {\it overconfidence\/} and {\it underconfidence\/} about the
posterior probability of cage A, {\it base rate bias\/} $(\beta_2 < \beta_1)$ resulting in
behavior consistent with the representativeness heuristic (i.e. excessive weight on the data via $\mbox{LLR}(n)$ relative
to the prior via $\mbox{LPR}(\pi)$), as well as conservatism ($\beta_2 > \beta_1$, i.e. putting excessive weight on prior
information relative to sample information).

Now consider the model of a subject's actual choice of cage A or B. We assume this choice depends on whether the
expected reward from choosing cage A exceeds the expected reward from choosing cage B, where the subject experiences
a reward $R$ if he/she selected the correct cage and 0 otherwise. We cast this decision as a binary choice that also
depends on idiosycratic noice terms $\epsilon=(\epsilon(A),\epsilon(B))$ that are independently distributed with  Type 1 extreme value distributed
marginal with scale parameter normalized to 1. While the subject observes when making their choice, the experimenter does not
so their decision will appear probabilistic from the experimenter's perspective. Let $d(\pi,n,\epsilon)$ be the subjectively
optimal decision rule of the subject
\begin{equation}
      d(\pi,n,\epsilon) = \left\{ \begin{array}{ll} A & \mbox{if} \quad  R\Pi_s(A|\pi,n,\beta) +\sigma\epsilon(A) \ge  R\Pi_s(B|\pi,n,\beta) 
+\sigma\epsilon(B) \cr 
    B & \mbox{otherwise}.
\label{eq:dr}
\end{array}
\right.
\end{equation}
As is well known from the discrete choice literature (see e.g. \citet{McFadden1974}) the probability that the subject chooses
cage A is given by the binomial logit formula
\begin{eqnarray}
   P(A|\pi,n,\beta,\sigma) &=& Pr\{ d(\pi,n,\epsilon)=A|\pi,n\} \nonumber \\
& =& { \exp\{R \Pi_s(A|\pi,n,\beta)/\sigma\} \over
 \exp\{R \Pi_s(A|\pi,n,\beta)/\sigma\} +  \exp\{R \Pi_s(B|\pi,n,\beta)/\sigma\}} \nonumber \\
    &=& { 1 \over 1 + \exp\{ R[1-2\Pi_s(A|\pi,n,\beta)]/\sigma\}}.
\label{eq:structural_logit}
\end{eqnarray}
It follows that when $\Pi_s(A|\pi,n,\beta)=1/2$ the subject is indifferent between choosing cage A or B and the noise
terms determine the actual outcome, resulting in a probability of choosing A that is also equal to 1/2. However as $\Pi_s(A|\pi,n,\beta)$
approaches 0 or 1, the ``strength of the evidence'' diminishes the role of the idiosyncratic shocks on the subject's choice,
and $P(A|\pi,n,\beta,\sigma) \to 1$ if $R$ is sufficiently large or $\sigma$ is sufficiently small and $P(A|\pi,n,\beta,\sigma) > 1/2$
and conversely $P(A|\pi,n,\beta,\sigma) \to 0$ when $P(A|\pi,n,\beta,\sigma) < 1/2$.

Notice that that the structural logit model results in a ``mixed strategy'' for the choice of bingo cage due to the 
effect of the idiosyncratic shocks $\epsilon$. However as $\sigma \to0$
it converges to a pure strategy that chooses cage A if $\Pi_s(A|\pi,n) \ge 1/2$ and cage B otherwise. Further if $\beta=(0,-1,-1)$
so the subjective posterior beliefs coincide with the true Bayesian posterior belief, then the structural logit model encompasses
the optimal pure strategy Bayesian decision rule $P^*(A|\pi,n)$ given in equation (\ref{eq:optpure}) as a 
special case.\footnote{\footnotesize \label{footnote:structural_probit} \citet{EGG1999}
introduced a three parameter {\it structural probit model\/} which is a decision rule
of the form $P(A|\pi,n,\beta)=\Phi(\beta_0+\beta_1\mbox{LLR}(n)+\beta_2\mbox{LPR}(\pi))$ where
$\Phi$ is the standard normal CDF. The optimal Bayesian decision rule $P^*(A|\pi,n)$ is not
nested within this class of models, though it can be approximated arbitrarily well in the limit
when $\beta_0=0$ and $\beta_1=\beta_2=\beta > 0$ and $\beta \to \infty$.}  

There are several ways to interpret the ``noise terms'' $\epsilon$ entering the subject's decision rule $d(\pi,n,\epsilon)$
in equation (\ref{eq:dr}). One is that they reflect momentary  distractions  that lead  to a certain element of randomness
in a subject's choice. Another interpretation is that it represents {\it calculational errors\/} in transforming the
information $(\pi,n)$ into a numerical subjective posterior belief $\Pi_s(A|\pi,n)$. The structural logit model (\ref{eq:structural_logit})
can also be derived from the assumption that due to calculational errors, the actual subjective posterior that
the subject experiences equals the true value $\Pi_s(A|\pi,n)$ plus an additive logistically distributed error term  with
mean zero and scale parameter $\sigma$. 

The structural logit choice probability $P(A|\pi,n,\beta,\sigma)$  will generally lie strictly inside the unit interval
so it results in a non-degenerate statistical model that enables us to estimate the unknown parameters $\theta=(\beta,\sigma)$
by maximum likelihood. We use a panel likelihood function since each subject $s$ in the experiment participates in 
a total of $T_s$ independent trials, so we observe a sequence of binary classifications $d_{ts}$ and corresponding
controls $(\pi_{ts},n_{ts})$ for each subject $s$ over trials $t=1,\ldots,T_s$. Note that the structural logit also
has an interpretation as a simple two layer feedforward neural network that processes two transformed inputs
$(\pi,n) \to (\mbox{LPR}(\pi),\mbox{LLR}(n))$ and has one hidden layer whose output is the subjective posterior  belief
$\Pi_s(A|\pi,n,\beta)$ and an output layer that takes the subjective posterior as its input and outputs a probability
of selecting cage A, $P(A|\pi,n,\beta,\sigma)$. Maximum likelihood can
be interpreted as ``training the neural network to behave like a human being.'' The ability of the structural logit model to fit a wide range of
subject behaviors can be ascribed to the flexibility afforded by using a parsimoniously parameterized neural network to
predict subject behavior.\footnote{\footnotesize The reader may consider it to be ``cheating'' to pre-transform the inputs
$(\pi,n)$ into $(\mbox{LPR}(\pi),\mbox{LLR}(n))$, since it is not clear that human subjects would actually make decisions based on any such transformation.
However additional layers can be added to the neural network so that the inputs to the extended network can be
$(\pi,n)$ and the first several layers can be interpreted as making the transformation of $(\pi,n)$ into
$(\mbox{LPR}(\pi),\mbox{LLR}(n))$ that feed into the two layer neural net we have developed as the the top two layers. We find
that these deeper networks
 have far many more parameters, but do not result in substantially better predictions of subject behavior than our
parsimonious 4 parameter two layer neural network specification. Indeed we can ``train'' our 4 parameter neural
network specification to behave nearly identically to a perfect Bayesian decision maker using training samples
with only a few dozen observations.}

The decision rule (or CCP) $P(A|\pi,n,\theta)$ can be used to form a likelihood so the parameters of the model
$\theta$ can be estimated by maximum likelihood. Let $S$ be the total number of subjects and suppose that each
subject $s$ participates in a total of $T_s$ trials in the experiment. Let $d_{ts}$ be the classification
reported by subject $s$ in trial $t$: $d_{ts}=1$ if subject $s$ chose cage
A and $d_{ts}=0$ if the subject chose cage B. The likelihood $L(\theta)$ is given by
\begin{equation}
     L(\theta) = \prod_{s=1}^S \prod_{t=1}^{T_s} P(A|\pi_{ts},n_{ts},\theta)^{d_{ts}}[1-P(A|\pi_{ts},n_{ts},\theta)]^{1-d_{ts}}.
\end{equation}
We estimated the El-Gamal and Grether model and the structural logit model for 221 of the 247 subjects reported
in \citet{EGG1995}.\footnote{Due to a corrupted data file we were unable to include 26 subjects from Pomona Community College
under the incentivized design where subjects were paid for a correct answer.} The results are shown graphically
in figure~\ref{fig:california_experiments} which compare predicted subject choices for several different
models and subsamples. In both panels, we plot the of  fraction of subjects choosing
cage A (y axis) as a function of the true Bayesian posterior probability of cage A (x axis). The black lines
in both panels are the actual fraction of the 221 subjects who chose cage A in the different trials of the
experiment where the values of the ``treatment variables'' $(\pi,n)$ are binned so we can plot results
on a two dimensional graph with the Bayesian posterior probabilities, $\Pi(A|\pi,n)$, on the x-axis.
Similar to figure~\ref{fig:humans_vs_robots} the dashed blue line represents the optimal decision rule of a perfect
Bayesian decision maker.  

\begin{figure}[ht]
\caption{Comparison of subject behavior and models in the Calfornia experiments}
\label{fig:california_experiments}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/ca_experiments_pay_vs_nopay-eps-converted-to.pdf}}\hskip .05in
\includegraphics[height=2.5in]{figs_pdf/structural_logit_vs_egg_model.pdf}}
\end{figure}

The left panel illustrates the effect of the incentive payments on subject behavior (blue curve for the no-pay
subjects, red for the subjects who were paid) and it is evident that it has negligible effect on overall
behavior.\footnote{We also plotted CCPs based on data from the first third of the trials with the last third
of the trials to see if there were any substantial ``learing by doing'' or ``experience effects'' and these
two were negligible.} The maximum likelihood predictions from El-Gamal and 
Grether's model of subject choice are the green curves in both panels. We see that this model fails to
fit the data well, particularly for $(\pi,n)$ values with a Bayesian posterior probability near $1/2$. This
pattern of prediction errors follows from their assumption about subject behavior already discussed, namely
that with probability $\varepsilon=.38$ subjects randomly guess a cage otherwise with probability $1-\varepsilon=.62$
they follow Bayes Rule. This  implies a discontinuous jump in the predicted probability of selecting cage A
right at $\Pi(A|\pi,n)=1/2$ since at that point the 62\% of subjects who are choosing according to Bayes Rule
jump from choosing cage B to choosing cage A.

The right hand panel of figure~\ref{fig:california_experiments} plots the predictions from
the structural logit model (red curve) as well as several ``reduced form'' models: 
1) a binary logit model with 3 parameters (for a constant, coefficient of $\pi$ and coefficient of $n$),
and 2) a 5 parameter two layer neural network that
includes an additional bias parameter in the upper output layer. We can see visually that the structural logit
model fits the data significantly better than the El-Gamal and Grether model even though both models have
4 parameters.  The El-Gamal and Grether model restricts 3 of the parameters, the cutoffs $c_\pi$, to a finite grid of integers, 
which allow far less flexibility in fitting the data compared to the 4 continuous parameters of the stuctural logit. The structural logit also
outperforms the 3 parameter reduced form logit (which can be regarded as a single layer feedforward neural network), but
produces approximately the same predictions as a 5 parameter neural network specification. The
structural logit model can be viewed as a restricted 4 parameter version of the 5 parameter neural network
where the bias term in the output layer is restricted to be -1/2  times the value of the input weight parameter, which is
$1/\sigma$ in the notation of the structural logit model. Intuitively, the structural logit model imposes a harmless
restriction that subjects compare their subjective posterior $\Pi_s(A|\pi,n)$ to the value 1/2 as the threshold for choosing  
cage A, and in particular, the restriction implies that subjects are equally likely to choose cage A or B when $\Pi_s(A|\pi,n)=1/2$.

\begin{table}[htbp]
\caption{Log-likelihood values for alternative models of subject choices}                                                                       
\begin{center} 
\label{tab:llf_california2}
\fontsize{11pt}{11}\selectfont
        %\label{tab:llf_california2}
        \setlength{\tabcolsep}{2pt}
        \renewcommand{\arraystretch}{1.15}
                \begin{tabular}{|l|c|c|c|} 
                        \hline
{\bf Model} & {\bf Number of parameters}& {\bf Log-likelihood} & {\bf AIC} \\
\hline
El-Gamal/Grether discrete cutoff rule & 4 &  -1952 & 3912 \\
\hline
Structural probit & 3 & -1847 & 3700 \\
\hline
Reduced-form logit  & 3&  -1821 & 3648 \\
\hline
Noisy Bayesian & 1 & -1801 & 3604 \\
\hline
Structural logit & 4 & -1773 & 3554 \\ 
\hline
Neural network & 5 & -1772 & 3554 \\
\hline
\end{tabular}
\end{center}
\end{table}

Table~\ref{tab:llf_california2} summarizes the fit of the various models of subject behavior. The final column
of the table reports the Akaike Information Criterion (AIC) used for model selection
and  defined as $2(k-LL)$ where $k$ is the number of parameters in the model and $LL$ is the maximized
value of the log-likelihood function for that model. Though the 4 parameter
El-Gamal and Grether model is not nested as a special case of the 4 parameter structural logit model, using the non-nested
likelihood-based specification test of \citet{Vuong1989} we can strongly reject the El-Gamal and Grether model in favor
of the structural logit model (P-value $2.5e-04$). Similarly, we can strongly reject the 3 parameter structural probit
(see footnote~\ref{footnote:structural_probit}) and the 3 parameter reduced form logit model as well (P-values $1.1e-06$ and $2.0e-05$ respectively ).
The noisy Bayesian model is a restricted 1 parameter version of the structural logit model where we allow $\sigma$ to be freely
estimated and restrict $\beta$ to impose Bayesian beliefs, i.e. $(\beta_0,\beta_1,\beta_2)=(0,-1,-1)$. A likelihood
ratio test strongly rejects the hypothesis that subjects are ``noisy Bayesians'' (P-value $9.2\times 10^{-12}$). 
The structural logit model is a restricted version of the 5 parameter neural network model and a likelihood
ratio test fails to reject the implicit upper level restriction on the bias term  discussed above. (P-value $.115$).
Overall, the structural logit model achieves the lowest value of the AIC (the same as the 5 parameter neural network
model) and it is another compelling reason why we use it as the preferred model for our subsequent analysis.

\begin{table}[htbp]
\caption{Maximum likelihood estimates of the structural logit/probit model parameters}                                                
\begin{center} 
\label{tab:sl_california_ml_estimates2}
\fontsize{11pt}{11}\selectfont
        %\label{tab:sl_california_ml_estimates2}
        \setlength{\tabcolsep}{2pt}
        \renewcommand{\arraystretch}{1.15}
                \begin{tabular}{|l|c|c|c|c|} 
\multicolumn{5}{c}{Structural logit model} \\
\hline
Parameter & $\sigma$  & $\beta_0$ &  $\beta_1$ & $\beta_2$ \\
                        \hline
Estimate &  .38  &  -.05  & -2.38   &   -1.86     \\
\hline
Standard error &  (.02)   &  (.05) &  (.28) &  (.19) \\
                 \hline
\multicolumn{5}{c}{Structural probit model} \\
\hline
Parameter & $\sigma$  & $\beta_0$ &  $\beta_1$ & $\beta_2$ \\
                        \hline
Estimate &  1  &  .03  & 1.05   &   .97     \\
\hline
Standard error &  (0)   &  (.02) &  (.04) &  (.04) \\
\hline
                \end{tabular}%
\end{center}
\end{table}

Table~\ref{tab:sl_california_ml_estimates2} presents the maximum likelihood coefficient estimates for the
structural logit model. Since the coefficient on $\mbox{LLR}(n)$, $\beta_1$ is significantly more negative
than the coefficient on $\mbox{LPR}(\pi)$, $\beta_2$, the estimation results suggests the typical subject
in El-Gamal and Grether's California experiments display the representativeness heuristic, contrary to
their finding that the single best model to predict subject behavior is the ``noisy Bayesian'' model (though
defined in terms of their threshold rule $c=(4,3,2)$ that corresponds to Bayes Rule).
We note that these initial results have ignored subject heterogeneity and assume all subjects are of a single type.
Later we will show how our conclusions change when we allow for unobserved heterogeneity in subjects' beliefs
and behavior.




\subsection{Identification of  Beliefs}

Now a few remarks on the identification of the parameters of the model, particularly the question 
as to whether it is possible to infer subjects' beliefs using only binary classification
data. First, we observe that it is impossible to separately
identify the reward $R$ and the error or noise parameter $\sigma$ since it 
is obvious from formula (\ref{eq:structural_logit}) that these parameters only appear together as a  ``signal to noise ratio''
$R/\sigma$ in the decision rule which in turn is used to form the likelihood for the data.  
Thus,  we assume that the reward $R$ from making a correct
decision is known (e.g. it equals the \$10 bonus for picking the correct cage). However in many case payoff may be in utility terms
and not directly known. 

In light
of this, in the subsequent analysis we normalize the payoff $R=1$ and estimate $\sigma$ subject to this normalization. However we must
keep in mind that a small estimated value of $\sigma$ may not necessarily indicate ``small noise'' in the subject's decision making
if the payoff from a correct answer, $R$, is sufficiently high. As we noted previously, similar to \citet{EGG1995} we do find
that the estimated value of $\sigma$ is lower in the incentivized experiments where subjects received a \$10 bonus
if they correctly selected the cage in a randomly selected trial  than in the ``no pay'' experiments. The lower estimated $\sigma$
probably reflects the higher reward and not that subjects' choice are necessarily less affected by idiosyncratic noise 
in the incentivized experiments.

An important question is whether the estimated structural logit model provides accurate estimates of
subjects' posterior beliefs, something we do not directly observe in the El-Gamal and Grether experiments.
Our's is an exercise in {\it revealed beliefs\/} where we attempt to uncover subjective posterior beliefs
from observations of subject's binary choices. In fact in the case where $\sigma=0$, we already have an identification
problem in that there are a continuum of non-Bayesian posterior beliefs that are consistent with the optimal
Bayesian decision rule $P^*(A|\pi,n)$.  To see this consider a family of beliefs indexed by a single parameter $\lambda > 0$
given by $\beta_\lambda=(0,-\lambda,-\lambda)$. It is not hard to show that for any $\lambda$ we have for any 
pair $(\pi,n)$
\begin{equation}
  \Pi(A|\pi,n) \le 1/2  \iff  \Pi_s(A|\pi,n,\lambda) \le 1/2,
\label{eq:iff}
\end{equation} 
and this condition implies that the implied decision rule for the subject coincides with the optimal
Bayesian decision rule $P^*(A|\pi,n)$ given by formula (\ref{eq:optpure}) even though the subject's posterior
beliefs are not Bayesian: they reflect ``underconfidence'' when $\lambda > -1$ and ``overconfidence'' when $\lambda < -1$ 
(i.e. an overconfident subject believes cage A is less likely compared to a Bayesian when $\Pi(A|\pi,n) < 1/2$
and  believe cage A is more likely than what  a Bayesian believes when $\Pi(A|\pi,n) > 1/2$).  We record this observation as

\begin{lemma} {\bf Non-identification of subject beliefs when $\sigma=0$}
\label{lemma:two}
When $\sigma=0$, a subject's beliefs cannot be identified from knowledge of the decision rule $P(A|\pi,n)$ they use, where the latter
is identifiable given sufficient experimental data on a subject's choices. In particular, 
there is a one dimensional continuum of non-Bayesian beliefs $\{\Pi_s(A|\pi,n,\lambda)|\lambda > 0\}$ for which
the implied optimal decision rule coincides with the optimal decision rule of a Bayesian decision maker, $P^*(A|\pi,n)$
given in equation (\ref{eq:optpure}).
\end{lemma}

However we do have a positive result on identification of posterior beliefs when $\sigma > 0$.

\begin{lemma} {\bf Identification of subject beliefs when $\sigma>0$}
\label{lemma:three}
When $\sigma>0$, all four parameters of the structural logit model are identified,
so the individual's subjective beliefs can be identified from knowledge
of their decision rule $P(A|\pi,n)$, where the latter
is identifiable given sufficient experimental data on a subject's choices. 
\end{lemma}
The proof of Lemma~\ref{lemma:three} is in appendix~A.
In light of Lemma~\ref{lemma:two} we need to proceed cautiously in how we interpret the inferred subjective beliefs
from the structural logit model. Even though Lemma~\ref{lemma:three} provides a theoretical justification for the
identification of the model when $\sigma > 0$, in practice it can be hard to distinguish the decision rule of a Bayesian
posterior beliefs where $\sigma $ takes on relatively large values (i.e. a ``noisy Bayesian'') from  a decision rule of a
non-Bayesian who has a very small value of $\sigma$ but also the $\beta$ coefficients that are close to zero.

The weak identification of subjective posterior beliefs is illustrated in figure~\ref{fig:weak_identification}. The figure
plots the CCPs for two very different values of the structural parameters:  $\theta_1=(.2,0,-.8,-.8)$ and
$\theta_2=(.002,0,-.008,-.008)$, i.e. $\theta_2=\theta_1/100$. The left panel plots the subjective posterior
beliefs $\Pi_s(A|\pi,n)$ for these two different ``subjects'' and we can see that they are very different, both from each other and
from the true Bayesian posterior (the dashed 45 degree line). However the right hand panel shows that the 
resulting CCPs $P(A|\pi,n)$ are nearly identical. This example does not contradict our identification result, Lemma~\ref{lemma:three},
because we can see that $P(A|\pi,n,\theta_1) \ne P(A|\pi,n,\theta_2)$ but the differences are really only apparent
at extreme values such as when $\pi$ is close to 0 or 1. So even though the structural logit is ``technically identified''
as a theoretical matter, but in any practical sense it is only weakly identified.\footnote{\footnotesize One way to understand the
identification problem is to note that the structural probit model of \citet{EGG1999} discussed in
footnote~\ref{footnote:structural_probit} must be subject to a location scale normalization on its normally  distributed error term. 
As we discussed above in the structural logit model the extreme value scale parameter $\sigma$ only appears as a ratio
$R/\sigma$ where $R$ is the payoff for a correct classification. However even if we normalize $R=1$ and Lemma~\ref{lemma:three}
assures us that the structural logit CCP is not scale invariant in its 4 parameters $\theta$, it is {\it approximately scale invariant\/}
as shown in figure~\ref{fig:weak_identification}. However imposing an arbitrary normalization such as $\sigma=1$ has behavioral
implications, since it determines the probability of incorrect classifications at the extreme values for the prior
probability of choosing cage A, i.e. $\pi=0$ or $\pi=1$. Indeed, our proof of identification used the knowledge of these classification
error probabilities at $\pi=0$ and $\pi=1$ to identify $\sigma$. But in actual data sets we may not have sufficient
data at $\pi=0$ or $\pi=1$ and in such cases the identification of $\sigma$ and the entire parameter vector $\theta$ will be 
more tenous.}

\begin{figure}[ht]
\caption{Example of weak identification of subjective posterior beliefs}
\label{fig:weak_identification}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/differing_subjective_probabilities.pdf}}\hskip .05in
\includegraphics[height=2.5in]{figs_pdf/but_nearly_observationally_equivalent_choice_probabilities.pdf}}
\end{figure}

As a result, the focus of the empirical work in this section will be on the {\it optimality of subjects'
decision rules\/} (which are non-parametrically identified) not necessarily on whether their posterior beliefs are Bayesian. Condition 
(\ref{eq:iff}) can be viewed as a sufficient condition for optimality of the decision rule of a non-Bayesian subject
and it results in a test for a weaker form of Bayesian rationality: $H_o: \beta_0=0$ and $\beta_1=\beta_2$. If this latter
hypothesis is satisfied, then the subject will still be modeled as behaving like a  ``noisy Bayesian''  even though their posterior
beliefs are not Bayesian. Later, in section 4, we return to the question of learning subjective posterior beliefs
using experiments that directly elicit these beliefs from the subjects.

\subsection{Accounting for Unobserved Subject Heterogeneity}

The experimental data we received from \citet{EGG1995} and \citet{EGG1999} does not contain any covariates
for observable characteristics of the subjects in the experiment. The only observable heterogeneity that we
can control for is the particular school where the experiment was run, and there was some evidence that students
at the more selected schools (e.g. UCLA) had a higher fraction of subjects classified as Bayesian, and a lower
estimated probability of making random guesses. 

However there is undoubtedly additional heterogeneity in the decision rules that subjects are using, including
different thought processes (including subjective posterior beliefs) that affect their classification decisions. 
One possible way to account for this additional {\it unobserved heterogeneity \/} is {\it fixed effects\/} where
we estimate subject-specific parameter vectors. However with $S$ subjects observed over $T$ time periods, we have
$ST$ total observations but a total of $4S$ parameters in the structural logit model. The time dimension (i.e. number
of trials) is rather limited in the California experiments with $T \le 20$ for the subjects at the the various
universitiess. The natural way to do asymptotic approximations for purposes of statistical inference is to assume
that $T$ is fixed and small whereas $S$ is potentially large. However this rules out the use of fixed effects as
a reliable method for inference due to the well known {\it incidental parameters problem\/} \citet{KW1956}.

Instead we use a {\it random effects\/} approach to inferring unobserved subject heterogeneity, where following
\citet{KW1956} we posit a  {\it distribution\/} $\mu(\theta)$ of preference parameters in the popluation and attempt
to estimate it. Treating $\mu$ as an arbitrary
element of the space of all distributions over $\theta$ results in an infinite dimensional ``parameter space'' 
and the estimation problem can be ill-posed unless some restrictions are imposed. Following \citet{HS1984} we estimate
a finite mixture approximation to $\mu$ by maximum likelihood, treating this mixture as a {\it sieve\/} (i.e. an expanding
parametric family that increases with sample size $S$ and can eventually approximate any $\mu$ when $S$ and the
number of mixture components is sufficiently large). 

Let $K$ denote the number of unobserved types to be estimated, and $\theta=(\theta_1,\ldots,\theta_K)$ be the $4K \times 1$
vector of parameters of the ``mixed structural logit model'' and let $\lambda=(\lambda_1,\ldots,\lambda_K)$ be the corresponding
$K \times 1$ vector of population probabilities of each of the $K$ types. Then the mixed logit likelihood function, $L(\theta,\lambda)$
is given by
\begin{equation}
     L(\theta,\lambda) = \prod_{s=1}^S \left[ \sum_{\tau=1}^K \lambda_\tau 
\prod_{t=1}^{T_s} P(A|\pi_{ts},n_{ts},\theta_\tau)^{d_{ts}}[1-P(A|\pi_{ts},n_{ts},\theta_\tau)]^{1-d_{ts}}\right].
\label{eq:hs}
\end{equation}
We estimate a sequence of such models starting with $K=1$ and increasing the number of types $K$ until a log-likelihood ratio test
is unable to reject a model with $K$ types in favor of a model with $K+1$ types, or alternatively,  picking the value of
$K$ for which AIC is minimized. 

We also estimate a closely related random effects approach called the {\it Estimation-Classification\/} (EC) algorithm
by \citet{EGG1995}. This algorithm also maximizes a likelihood function but instead of computing a mixture over
types for each subject as in equation (\ref{eq:hs}) the EC algorithm {\it assigns each subject in the sample their most
likely type.\/} That is, the EC algorithm is the $4K\times 1$ vector $\theta=(\theta_1,\ldots,\theta_K)$ together with the 
$S \times 1$ vector of maximum likelihood subject classifications $\tau=(\tau_1,\ldots,\tau_S)$ where $\tau_s$
denotes the most likely type for subject $s$. That is, we can write the EC estimator $(\hat\theta,\hat\tau)$ as the 
pair $(\theta,\tau)$ that maximizes the following likelihood
\begin{equation}
     L(\theta,\tau) = \prod_{s=1}^S \left[ \sum_{k=1}^K I\{\tau_s=k\} 
\prod_{t=1}^{T_s} P(A|\pi_{ts},n_{ts},\theta_k)^{d_{ts}}[1-P(A|\pi_{ts},n_{ts},\theta_k)]^{1-d_{ts}}\right].
\label{eq:ec}
\end{equation}
Thus, the Heckman-Singer finite mixture estimator can be conceptualized as a ``mixed strategy'' since it 
treats each subject as a mixture over $K$ possible types, whereas the EC estimator can be regarded as
a ``pure strategy'' since instead of using a mixture over types, it assigns each subject their most likely type. 
The EC algorithm results in the following implied mixture probabilities,
\begin{equation}
         \hat\lambda_k = \frac{1}{S} \sum_{s=1}^S  I\{\hat\tau_s=k\},
\end{equation}
i.e. $\hat\lambda_k$ is simply the fraction of subjects whose most likely type is $k$. Similar to the finite
mixture estimator, we use the same sequential procedure to identify the number of types $K$ by starting with $K=1$ and
sequentially increasing $K$ until a likelihood ratio test fails to reject the hypothesis that a model with $K$
types fits significantly better than a model with $K+1$ types, or alternatively we can pick the value of $K$ with the smallest AIC.


\subsection{Reanalysis of Wisconsin Experiments}

We now turn to a reanalysis of the data from the ``Wisconsin experiments'' conducted
by \citet{EGG1999}. They recruited a total of 79 student subjects from the University of Wisconsin-Madison
and employed an innovative two stage experimental design to test for {\it context effects\/} by altering
the ``California design'' used in \citet{EGG1995} (which involved drawing 6 balls with replacement
from bingo cages containing 6 balls each) to a new ``Wisconsin design'' that involved drawing 7 balls
with replacement from bingo cages containing 10 balls each. Further, they altered the fractions of balls
marked N and G in the Wisconsin design, using the values $p_A=.4$ and $p_B=.6$, respectively.  The reason
this was done was twofold: 1) by drawing an odd number of balls, they made it harder for subjects to rely
on the ``representativeness heuristic'' in their choice of cage A or B, and 2) by reversing the proportions of
balls marked N they reversed the classification rules. That is, in the 7 ball Wisconsin design a larger number $n$ of balls marked
N in the sample constitutes stronger evidence for cage B, not cage A as was true in the California design.
The Wisconsin experiments were conducted
on two successive days. On the first day approximately half the subjects were started with the 6 ball California
design and then switched to the 7 ball Wisconsin design on the second day, whereas the other half of subjects
this order was reversed. This was done to check if the ordering of the designs had any effect on subjects' choices.

From our perspective, the Wisconsin experiments provide an opportunity to treat the switch from the 6 ball California
design to the 7 ball Wisconsin design as a {\it policy change\/} to study how well the structural logit model
is able to predict subjects' choices under a different experimental design (data generating mechanism). Thus, we estimate a multi-type
version of the structural logit model for all 79 subjects using the 6 ball California design trials as the
{\it training sample\/} and the the 7 ball Wisconsin design trials as the {\it evaluation sample.\/} This approach
also allows us to conduct a likelihood ratio test for {\it structural stability,\/} i.e. do the subjects use the
same classification decision rule in both designs, or  do they appear to use different decision rules across
successive days of the experiment? As we noted in the introduction, \citet{EGG1999} concluded (using their structural
probit model) that subjects did appear to use different decision rules in the 6 ball and 7 ball designs. Evidently  not
being able to rely as easily on the representativeness heuristic lead a greater fraction of subjects to use
decision rules that more closely approximate a noisy version of Bayes rule in the 7 ball trials.

Figure~\ref{fig:wisconsin_experiments} plots the raw data on subject choices in both the 6 and 7 ball trials
in the Wisconsin experiments. The size of each circle is proportional to the number of observations and the color
of the circles represents the share of subjects choosing cage A or B. Thus, deep blue circles are those where
nearly all of the subjects chose cage B, deep red circles are those where nearly all the subjects chose cage A,
and the purple colored circles are those where there was a mix of subjects choosing cage A and B. We mixed
the colors red and blue to color each circule with the same proportion as the fraction of subjects choosing A and B.


\begin{figure}[ht]
\caption{Data and classification thresholds in the Wisconsin experiments}
\label{fig:wisconsin_experiments}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/california_design_and_raw_data.pdf}}\hskip -.15in
\includegraphics[height=2.5in]{figs_pdf/wisconsin_design_and_raw_data.pdf}}
\end{figure}

To help assess whether subjects' responses are consistent with the optimal Bayesian decision rule, the
black lines in each figure show the {\it classification hyperplane\/} i.e. the dividing line between points
where a Bayesian would choose cage A and the points where the Bayesian would choose cage B. Specifically,
the black lines graph the set of points $(\mbox{LLR},\mbox{LPR})$ that satisfy the equation
\begin{equation}
            \mbox{LLR} + \mbox{LPR} = 0,
\label{eq:bayesian_hyperplane}
\end{equation}
which is mathematically equivalent to the indifference condition $\Pi(A|\mbox{LLR},\mbox{LPR})=1/2$ where a Bayesian
is just indifferent between choosing cage A or B. For other lines (not plotted) if $\mbox{LLR}+\mbox{LPR} > 0$ then the
Bayesian would strictly prefer to choose cage A and the magnitude of this sum can be viewed as an index of 
a Bayesian's ``strength of belief'' that cage A is the correct one. That is, as $\mbox{LLR}+\mbox{LPR} \to \infty$
we have $\Pi(A|\mbox{LLR},\mbox{LPR}) \to 1$, and vice versa when $\mbox{LLR}+\mbox{LPR} < 0$.
We see from the figures that indeed, subjects are rather ``confused'' (indicated by purple colored circles) for trials where 
$(\mbox{LLR},\mbox{LPR})$ lies near the black classification hyperplane or ``indifference curve'' but the circles further
away from it are colored deep red or blue, so subjects are in strong agreement and are making classifications
in accordance with Bayes Rule.

Table~\ref{tab:sl_wisconsin_ml_estimates2} presents the maximum likelihood estimates using the EC algorithm
of \citet{EGG1995} to estimate the 4 parameter structural logit model.\footnote{\footnotesize Estimation results
using a finite mixture specification are very similar and are presented in Appendix XX along with results
for multitype models estimated using the 221 subjects in the California experiments.}  We stopped the EC algorithm when it reached
$K=3$ types even though the likelihood ratio test indicated that $K=4$ types is a significantly better fit because
with only 79 subjects, there would be too few subjects assigned to some of the types in the 4 type model, raising
the possibility of model overfitting and less reliable inferences. 

\begin{table}[htbp]
\caption{EC estimates of the structural logit model with 3 types of subjects, $LL=-654.25$}                                                
\begin{center} 
\label{tab:sl_wisconsin_ml_estimates2}
\fontsize{11pt}{11}\selectfont
    %\label{tab:sl_wisconsin_ml_estimates2}
        \setlength{\tabcolsep}{2pt}
        \renewcommand{\arraystretch}{1.15}
                \begin{tabular}{|l|c|c|c|} 
\hline
Parameter (std error) & Type 1 ($\hat\lambda_1=.32$)  & Type 2 ($\hat\lambda_2=.24$) & Type 3 ($\hat\lambda_3=.44$)  \\
\hline
$\sigma$ (noise parameter) & .07         & .22   & .32 \\
                           &       (.08) & (.06) & (.05) \\
\hline
$\beta_0$ (bias/intercept) & -.14        & -.06  & .11 \\
                           & (.18)       & (.11) & (.08) \\
\hline
$\beta_1$ ($\mbox{LLR}(n)$ coefficient) & -1.48 & -1.25 & -2.48 \\
                                     & (1.91)& (.36) & (.67) \\
\hline
$\beta_2$ ($\mbox{LPR}(\pi)$ coefficient) & -1.40 & -2.27 & -1.39 \\
                                     & (1.81)& (.70) & (.36) \\
\hline
$P$-value for $H_o: \beta_0=0,\beta_1=\beta_2$ & .74 & .02 & .01 \\
\hline
$P$-value for $H_o: \beta_0=0,\beta_1=\beta_2=-1$ & .015 & .003 & .015 \\
\hline
\end{tabular}%
\end{center}
\end{table}

Of the three types, type 1 is the most ``Bayesian'' and also the least ``noisy''. The estimated noise parameter
$\sigma$ is less than a third of the value estimated for the other two types.  There is no significant overall
bias in the beliefs of any of the three types as evidenced by the fact that all three estimates of the 
bias term $\beta_0$ in $\Pi_s(A|\pi,n,\beta)$ (i.e. the constant term in equation~(\ref{eq:subjectiveposterior})
is insignificantly different from zero. The next to the last row in the table presents the P values
of a Wald hypothesis test that $\beta_0=0$ and $\beta_1=\beta_2$, and we see that there is no evidence against
this for type 1 subjects but the hypotheis is rejected for type 2 and type 3 subjects. The latter subjects
can be described as type R and C, respectively where type R subjects are those whose beliefs are consistent with the Representativeness
heuristic and who put less weight on the prior information via $\mbox{LPR}(\pi)$ relative to the sample information
via  $\mbox{LLR}(n)$. Conservative subjects do the opposite, putting higher weight on $\pi$ than
on $n$. 

However the last row of the table shows that we can strongly reject the hypothesis that any of the three types are ``noisy Bayesians'' i.e.
who satisfy the hypothesis $H_o: \beta_0=0, \beta_1=-1, \beta_2=-1$,  though with possible noise affecting their choices, $\sigma > 0$. 
But because the type 1 subjects satisfy the restriction that $\beta_0$ and $\beta_1=\beta_2$, their implied decision rule
is nearly optimal, as we show below. So at least in terms of their decision rule or {\it choice behavior\/} the type 1 subjects
are close to optimal  even if their subjective posterior beliefs may be a distorted version of true Bayesian beliefs.
Figure~\ref{fig:posterior_beliefs} plots the estimated subjective posterior beliefs for the three types of subjects (dotted lines)
and compares them to the true Bayesian beliefs (solid lines) for all possible combinations $(\pi,n)$ where $\pi \in [0,1]$ and
$n \in \{0,1,\ldots,6\}$. 


\begin{figure}[ht]
\caption{Subjective vs Objective Posterior Beliefs}
\label{fig:posterior_beliefs}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/type1_subjective_posterior_vs_bayes_posterior.pdf}}\hskip -.15in
\includegraphics[height=2.5in]{figs_pdf/type2_subjective_posterior_vs_bayes_posterior.pdf}}
\centerline{\includegraphics[height=2.5in]{figs_pdf/type3_subjective_posterior_vs_bayes_posterior.pdf}}
\end{figure}

It is readily apparent visually that the subjective posterior beliefs of the Type 1 subjects are closest
to Bayesian, but there are clear distortions in the estimated posterior beliefs for the Type 2 (R) and Type 3 (C)
subjectss. The type R subjects display a pattern of {\it overconfidence\/} by overestimating the probability
of A relative to Bayes Rule for sufficiently high values of $\pi$ and under-estimating it for sufficiently low
values of $\pi$. The type C subjects suffer from a different type of overconfidence. For high values of $n$
($n \in \{0,1,2,3\}$) these subjects have subjective beliefs that systematically under-estimate the probability
of A relative to Bayes Rule for {\it all\/} values of $\pi$, but for high values of $n$ ($n \in \{5,6\}$) this reverses and they systematically
over-estimate the probability of A relative to Bayes Rule, again for all values
of $\pi \in [0,1]$. 

These distortions in subjective posterior beliefs lead to suboptimal choices even
in the absence of ``noise'' in their ultimate decisions. If $\sigma$ were zero, the optimal decision rule
can be described by a {\it cutoff rule\/} $\overline\pi(n)$ that differs for each realized value of $n$, the
number of balls marked N in the sample of 6 balls. These cutoffs occur at the intersections of the solid or
dashed curves with a horizontal line at a probability value of $1/2$, so that is it optimal for the subject
who observes information $(\pi,n)$ to choose cage B if $\pi < \overline\pi(n)$ and cage A if $\pi \ge \overline\pi(n)$.
From this it is evident that the Type 1 subjects have the least distortion the implied optimal (noise-free)
decision rules, whereas the Type 3 subjects have the most distorted decision rule. We will show below that
this translates directly into a significantly higher loss for type 3 subjects relative to type 1 subjects.

Before illustrating this, we first present figure~\ref{fig:fraction_of_optimal_responses}
which plots, for each of the 79 subjects in the experiment, the fraction of ``correct'' responses, i.e. the fraction
of their responses that coincide with the optimal choice a perfect Bayesian decision maker would make given
the same information $(\pi_t,n_t)$ in each trial $t$. We see that the fraction of correct responses ranges from a
low of 54\% to a high of 100\% with an average of 81\% correct responses over all 79 subjects. To relate ``correctness''
to Bayesian behavior the figure plots the posterior probability that each subject is a type 1 ``noisy Bayesian'' subject
and the solid red curve shows the results of a local linear regression showing the local average probability that the
subjects (ordered by percent of answers correctly answered) is a ``noisy Bayesian''.  As expected there is a positive
relation between ``correctness'' and the probability of being a Type 1 subject, ranging from a low of 0\% for 
subjects who only managed to answer 54\% of the trials correctly to a high of 70\% for subjects who answered 100\% correctly.
Of course, it is possible to get 100\% correct via randomly guessing the right answer and this is why the posterior
probability of subjects who answered 100\% correctly is not 1.\footnote{\footnotesize In fact, the posterior probability
of being a Type 1 subject can be rather low even if the subject answered 100\% correctly depending on the particular
sequence of trial values $\{(\pi_t,n_t)\}$ the subject is asked to classify. If most of these trials correspond
to true posterior values close to 1/2, i.e. $\Pi(A|\pi_t,n_t) \simeq 1/2$, then chances are significantly higher that
the subject could have simply been guessing the right answers, and this substantially elevates the probability that
the subject could also have been a type 2 or 3 subject and got 100\% of the answers correct also, again via
random guessing.}

\begin{figure}[ht]
\caption{Fraction of Correct Responses}
\label{fig:fraction_of_optimal_responses}
\smallskip
\centerline{\includegraphics[height=3.0in]{figs_pdf/fraction_of_correct_responses.pdf}}
\end{figure}

Figure~\ref{fig:expected_loss_functions} plots the implied ``classification hyperplanes'' for each of the three
types of subjects along with the prior-specific expected loss functions $LP(\pi)$, see equation (\ref{eq:lossdef}), 
implied by the model estimates and the implied decision rules (CCPs) $P(A|\pi,n,\hat\theta_\tau)$, $\tau \in \{1,2,3\}$. 
The lines (hyperplanes) graph the pairs of points $(\mbox{LLR},\mbox{LPR})$ satisfying 
\begin{equation}
               0 = \hat\beta_{0,\tau}+ \hat\beta_{1,\tau}\mbox{LLR}+\hat\beta_{2,\tau}\mbox{LPR},
\end{equation}
for each estimated type and also the Bayesian posterior threshold $\mbox{LLR}+\mbox{LPR}=0$ for comparison. Recall
that along these lines the subject believes cages A and B are equally likely, so they each demarcate the 
decision regions each type of subject would make their classification decisions in the absence of noise (i.e. when $\sigma=0$).  Here it is
obvious that  the decision hyperplane of the Type 1 subjects essentially coincides with the Bayesian
classification hyperplane, but the hyperplane for the Type 2 subjects is significantly less steep
and the hyperplane for the Type 3 subjects is significantly more steep than the classification hyperplane
of a Bayesian. From this, we can readily assess the regions where subjects will make classification errors
relative to what an optimal Bayesian decision maker would choose. For example in the triangular region
to the left of $\mbox{LPR}(\pi)=0$ below the red and black lines and above the blue line, for values
of $(\mbox{LLR}(n),\mbox{LPR}(\pi))$ in this region a type 2 subject chooses cage A but a Bayesian (or type 1 subject)
chooses cage B. Similarly the triangular region below the green line and above the red and black lines
to the left of $\mbox{LPR}(\pi)=0$, represents suboptimal classifications by Type 3 subjects: they would
choose cage B whereas a Bayesian (or type 1 subject) would choose cage A. 

\begin{figure}[ht]
\caption{Classification Hyperplanes and Expected Loss Functions}
\label{fig:expected_loss_functions}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/estimation_classification_hyperplanes.pdf}}\hskip -.15in
\includegraphics[height=2.5in]{figs_pdf/expected_loss_functions.pdf}}
\end{figure}


The right hand panel of figure~(\ref{fig:expected_loss_functions}) plots the expected conditional loss function $L_p(\pi)$
(i.e. the conditional probability of predicting the wrong cage used to draw the sample conditional on an experiment
where $\pi$ is the prior probability of choosing cage A). The black curve plots $L_P(\pi)$ for a Bayesian
decision maker, and by Lemma~\ref{lemma:bayes_optimality} it must have the lowest loss compared 
to any other decision rule, so the black curve necessarily minorizes the expected loss curves for the
type 1, 2 and 3 subjects. However see that the red expected loss curve for the type 1 subjects nearly coincides
with the black Bayesian curve, indicating that the Type 1 subjects are nearly optimal Bayesian decision makers,
even if their subjective posterior beliefs are distorted relative to Bayes Rule.  However the green and blue curves
are significantly higher than the black and red expected loss curves, showing that the Type 2 and 3 subjects are using 
distinctly suboptimal decision rules. Most suboptimal decision makers are the type 3 subjects whose $L_P(\pi)$ loss
function majorizes the other three expected loss functions. Note that the other loss functions are close to zero
at values of $\pi$ equal to 0 or 1, but the green curve is significantly positive at those values. This is a refection
of the high amount of ``decision noise'' $\sigma$ for the type 3 subjects that we noted in our discussion of the
estimation results in table~\ref{tab:sl_wisconsin_ml_estimates2}. That is, a type 3 subject chooses cage A about 
5\% of the time even when there is $\pi=0$ chance that cage A will be selected, and conversely these subjects choose
cage B 5\% of the time when $\pi=1$ whereas a rational person should always choose cage A.

If we take an expectation of the $L_P(\pi)$ expected loss functions with respect to
some distribution $F(\pi)$ (i.e. a ``prior over priors'') we obtain a convenient single summary
index of the degree of of suboptimality of each subject, allowing us to provide an unambigous ranking of the
three types of subjects. We define the {\it relative inefficiency index\/} as the ratio $I=E\{L_P(\pi)\}/E\{L_{P^*}(\pi)\}$ 
of the unconditional expected loss implied by a decision rule $P$ to the minimized loss from an optimal
Bayesian decision rule $P^*$. The respective inefficiency indices for type 1, 2 and 3 subjects, respectively
are $I_1=1.01$, $I_2=1.09$ and $I_3=1.22$. We can also use the delta method to compute the standard errors
for these three inefficiency index ``point estimates'' and use a Wald test to see if we can reject the hypothesis
that the efficiencies of the three type of subjects are all equal to each other.

Finally, we consider the ability of the structural model to predict a ``policy change'' i.e. a change in the
experimental design from the 6 ball Calfornia design to the 7 ball Wisconsin design. We illustrate this in figure~\ref{fig:predicted_vs_actual}.
The left panel of the figure shows the in-sample fit, i.e. it compares the predicted CCPs  from the structural
model to the non-parametric estimates of the CCPs for subjects in the 6 ball ``training sample''. Note that we incorporated
the subject-specific unobserved heterogeneity in the model-predicted CCPs in this figure: that is, we  computed the 
structural logit CCPs by averaging the subject-specific CCPs where each subject was assigned their most likely
type from the output of the EC estimation algorithm.
We plot separate lines for the 4 separate priors used in these experiments, $\pi \in \{.3,.4,.6,.7\}$ where the dashed
lines plot the non-parametric CCPs as a function of $n$ and the solid lines are the preditions of the structural logit model.

\begin{figure}[ht]
\caption{Predicted vs Actual CCPs in Training and Evaluation Samples}
\label{fig:predicted_vs_actual}
\smallskip
\centerline{\includegraphics[height=2.5in]{figs_pdf/expected_vs_predicted_ccps_6ball_trials.pdf}}\hskip -.15in
\includegraphics[height=2.5in]{figs_pdf/expected_vs_predicted_ccps_7ball_trials.pdf}}
\end{figure}

The right hand panel illustrates the ability of the structural logit model to predict how subject behavior
changes in the ``evaluation sample''.  Notice that the 4 curves are now {\it downward sloping in $n$\/} and of course
this is due to a change in the proportions of N balls in each bingo cage: from $(p_A,p_B)=(2/3,1/2)$ in the California
design to $(p_A,p_B)=(.4,.6)$ under the Wisconsin design. As we already noted, this implies that higher values
of $n$ provide stronger evidence {\it against\/} the hypothesis that the sample came from cage A for any given prior.
We see that the structural logit model provides fairly accurate predictions of the dramatic shift in subjects'
decision rules under the two experimental designs, suggesting that the structural logit model provides a good approximation
to subject behavior. In particular, the structural logit model ``builds-in'' the implicit dependence of the three
experimental design parameters $(J,\pi_A,\pi_B)$ where $J$ is the number of balls drawn with replacement from the
chosen bingo cage, so $J=6$ for the California design and $J=7$ for the Wisconsin design. These ``experimental
controls'' or design parameters determine the binomial data generating mechanism that subjects
are confronting in the experiments and as such  
constitute critical additional information to be able to make a sensible decisions.
As we can see in the figure changing these controls significantly alters subject behavior and the structural logit model
accurately predicts how subjects' decision rules changed in the evaluation sample.


However there is a more subtle aspect in which subjects' decision rules might have changed  that constitutes
evidence against the ``structural stability'' of the structural logit model. That is, if the structural logit
model was a completely correct model of subject behavior, then if we were to estimate the parameters of the
structural logit model using the 7 ball evaluation sample, we should get results that are not significantly
different statistically from the parameters estimated in the 6 ball training sample.  However 
we find that that when we do use the 7 ball experiments as the estimation or
training sample,  there is a significant change in the structural parameter estimates: {\it now, a positive fraction
of subjects, 25\%,  can be classified as ``noisy Bayesians''.\/} However the noisy Bayesians also exhibit significantly
greater noise in their responses compared to the type 1 subjects when we estimated the
model using the 6 ball design as the training sample, with $\hat\sigma=.43$ and estimated error of $.15$.   

Overall, when we estimate the structural logit model using the 7 ball design as the training sample,
we find that type 1 and 3 subjects have relatively low inefficiency indices but type 2 subjects exhibit
high inefficiency due to the large values of $\sigma$ noted above. In the 7 ball data, we find that the inefficient, high noise
subjects constitute 25\% of the sample, whereas the other 75\% of subjects  have lower inefficiency due to
lower estimated values of $\sigma$. Overall the fraction of subjects using ``efficient'' decision rules increased from 32\% when we
used the 6 ball experiments as the training sample to 75\% when we used the 7 ball experiments as the training sample.  
Further, a likelihood ratio test strongly rejects the hypothesis that subjects were using the same decision rules
in both the 6 ball and 7 ball experimental designs: P-value $.002$.\footnote{\footnotesize When we estimated the
3 type structural model via EC using the 221 California subjects  we obtained roughly similar results as we obtained
for the Wisconsin subjects when we estimated their parameters for the same 6 ball ``California design''. We found
that 21\% of the California subjects were ``noisy Bayesians'', 50\% overweight $\mbox{LLR}(n)$ and hence show
behavior consistent with the representativeness heuristics, and 29\% overweight $\mbox{LPR}(\pi)$ and hence
exhibit behavior consistent with conservatism. However the noise estimated $\sigma$ parameter for the noisy Bayesian 
was $\sigma=.74$ and this high level of noise made the noisy Bayesian subjects by far the most suboptimally
behaving subgroup of the California subjects.}

We conclude by emphasizing the five main takeways from our reanalysis of human subject data from
\citet{EGG1995} and \citet{EGG1999}.

\begin{itemize}
\item[1.] We find substantial unobserved heterogeneity among different subjects as well as
significant idiosyncratic random noise that affects their responses.
\item[2.] Although some subjects {\it behave\/} approximately as optimal Bayesian decision makers, it is less clear
that their {\it beliefs\/} are close to Bayesian.
\item[3.] Since decision rules are well identified, we are confident in using the model
to classify subjects in terms of the degree of suboptimality in their decision making. We find
a minority of subjects behave close to the optimal Bayesian decision rule, but the majority 
exhibit significant inefficiencies, both from improper evaluation/processing of the evidence and 
also from random noise that affects their responses.
\item[4.] The structural logit model provides a good approximation to the different decision rules
used by different subjects in these experiments as well as good ``out-of-sample'' forecasts of how their
behavior changed under the ``Wisconsin design''.
\item[5.] However our analysis confirms the main conclusion of \citet{EGG1999}
 that there were additional changes in subject behavior
under the Wisconsin design that cannot be predicted by the structural logit
model  purely on the basis of the change in data generating
mechanism  parameters from the ``California design''. This suggests  that human subjects 
are affected by to {\it context effects\/} and may rely on heuristics such as the representativeness to reduce cognitive
burden when a heuristic is readily available (as in the California design) whereas when the heuristic 
is not obviously applicable (as in the 7 ball Wisconsin design) subjects did not appear to rely on it as much
and this  may explain why their behavior was better approximated as ``noisy Bayesian''
(though the level of noise affecting their responses also increased).
\end{itemize}

Conclusion 4 seems roughly consistent with the main hypothesis of \citet{Kahneman2011}  on two different
modes of human thinking, {\it System 1 and System 2.\/}  Some experimental designs
can encourage human subjects to rely more on ``System 1'' (the faster, more instinctual/intuitive subsystem he posits
humans rely on on a day to day basis to minimize cognitive burden) but in designs where simple
heuristics are not clear appropriate or applicable, human subjects may rely more on  ``System 2'' (the slower, more deliberative
and logical model of thinking but which requires more energy). However this is speculative, and all we can conclude
definitively from our analysis is that we can reject the hypothesis of {\it structural stability\/} across the
two experimental designs, i.e. that even though the data generating mechanism might change, the structural
parameters are unaffected by ``policy changes'' including changes in the experimental design that alter the
``data generating mechanism'' that subjects confronted under the 7 ball Wisconsin design.


==> 6_textual_analysis.tex <==
% analysis of textual responses

Most econometric models treat humans as black-boxes and apart from some research from neuroscience, we do not know exactly how humans process information. However, with GPTs we have the unique advantage of knowing both how their neural ``brains" compute information and the textual response which contains their reasoning behind their answers. Therefore, it makes logical sense to try to parse this text to understand how and why GPTs made mistakes, create a taxonomy of errors and obtain error distributions across models. However, there are some complications. There is more than one way to answer the question correctly and even more ways to make mistakes. The approach we adopted was twofold: (1) create a process for automated grading using a superior GPT model, and (2) manual grading of a smaller sample of GPT4o's responses. 

\subsection{Automated Grading of Textual Responses}

\subsubsection{Data and Methodology}

Due to inherent difficulties in scaling manual grading we came up with a novel algorithm to parse and process GPT's textual responses using a superior GPT model itself. A grading prompt was created which provided the original question, the original answer, the numerical values and logical process that a perfect answer would entail, and detailed instructions on how to mark and grade. After some pilots, we were able to identify 9 yes/no ``flags" that could be raised by a grader GPT in an objective way so as to reduce ambiguity and increase precision. The data consists of a balanced sample of 300 responses per model that were graded by the latest version of ChatGPT, o1, using this grading prompt. We present the error distributions identified by the flags that o1 created. The overall process can be seen in Algorithm~\ref{alg:grading}. 

\begin{algorithm}
\caption{Automated Grading by a Teacher GPT\label{alg:grading}}
\begin{algorithmic}[1]
\State Sample record from data obtaining Original Prompt and Student GPT's Response.
\State Compute an Ideal Answer (teacher's ideal) for each valid prompt-response pair.
\State Build a Grading Prompt combining Original Prompt, Original Response, and Ideal Answer.
\State Send each Grading Prompt to Teacher GPT to obtain a Grading Response.
\State Extract the evaluation flags from Grading Response and store results.
\end{algorithmic}
\end{algorithm}


Table \ref{tab:grading-flags} contains the flags which are categorized into themes. Broadly, we are asking the following questions, (a) did the GPT understand the question and the information present in it? (1-3) (b) did the GPT at least conceptually try to apply Bayes rule? (4-5) (c) did the GPT make numerical errors in calculation? (6-8) (d) did the GPT have any last second logical contradiction in its own reasoning (9)?.

\begin{table}[h!]
\centering
\caption{9-Part Grading Flags from Teacher GPT's Grading Response \label{tab:grading-flags}}
\begin{tabular}{p{1cm} p{4cm} p{9cm}}
\toprule
\textbf{Index} & \textbf{Flag (Yes/No)} & \textbf{Description} \\
\midrule
1 & Cage Composition & Are N vs.\ G compositions used correctly? \\
2 & Draw Count & Are total draws handled correctly? \\
3 & Observed Data & Is the observed outcome properly incorporated? \\
4 & Ignoring Prior & Is the prior probability completely omitted? \\
5 & Conceptual Bayes & Are both prior and likelihood conceptually combined? \\
6 & Prior Computed & Is the prior numerically computed? \\
7 & Likelihood Computed & Is the binomial coefficient applied correctly? \\
8 & Posterior Computed & Are posterior or posterior ratios computed? \\
9 & Inconsistency & Is there a final contradiction in the reported choice? \\
\bottomrule
\end{tabular}

\end{table}

All grading, including human grading, will contain noise, the question is if the noise is below some threshold. A small subset (2.5\%) 
of the grading was manually evaluated by us and we find an error rate of less than 2\%. After the grading we looked at the 
errors identified and manually checked to see if they made sense. There will be some errors that we may not be able to 
identify due to noise in the grading, but some cannot be explained away as statistical artifacts. 
This automation, though imperfect, is a scalable way to obtain error distributions and get a sense of what went wrong as the GPT tried to answer the question. We also try to map these flags to try to verify the structural logit model estimates, even though a perfect map is infeasible. 

\subsubsection{Reading and Writing Errors}

The first three questions (Flags 1, 2, and 3) address reading errors, which involve messing up total draws, cage compositions and observed data, as well as writing errors, which involve incorrectly parsing the question’s given data into formulas. We do not expect GPTs to make too many of these errors as one of their strengths is text parsing and text generation. Consistent  with that expectation we find that most models do not make reading and writing errors, but in rare cases this can happen, even in our leading models. 

\begin{tcolorbox}[breakable, title={GPT3.5 Mixes up the Cage Composition in Step 3}]
\singlespacing
Step 1: Calculate the probability of drawing 4 "N" balls and 3 "G" balls from each cage:
\begin{itemize}
    \item Cage A: \( \left(\frac{4}{10}\right)^4 \times \left(\frac{6}{10}\right)^3 \approx 0.0216 \)
    \item Cage B: \( \left(\frac{6}{10}\right)^4 \times \left(\frac{4}{10}\right)^3 \approx 0.0138 \)
\end{itemize}
Step 2: Compare the probabilities:
\begin{itemize}
    \item The probability for Cage A is higher.
\end{itemize}
Step 3: Note that Cage A has more "N" balls than Cage B.\\[1ex]
Final Decision: Cage A.
\end{tcolorbox}

The full error distribution is presented in Figure \ref{fig:read-write-errors}. The evidence suggests that GPT3.5 makes slightly more such errors than GPT4 or GPT4o and it appears that the one area where the error rate is slightly higher is using information regards the total draws. These types of errors are not part of the structural logit model, which assumes that base information is read correctly. Therefore, the finding that these errors happen very rarely is an indirect validation of the modelling choice of abstracting away from such errors. 

\begin{figure}[h!]
    \centering
    \caption{Average Reading and Writing Errors by Model (Mean ± SE) (N=1200)}
    \includegraphics[width=1.0\linewidth]{figs/text1.png}
    
    \label{fig:read-write-errors}
\end{figure}

\subsubsection{Conceptual and Knowledge Errors}

The next two flags (4 and 5) try to pin down if the response correctly applied Bayes rule, or alternatively made a decision based on the likelihood or priors alone. This question explicitly ignores any numerical considerations and focused squarely on conceptual application. 

\begin{tcolorbox}[breakable, title={GPT4o Decision based on Likelihood Only (Edited for Brevity)}, fontupper=\footnotesize]
Step 1: Compute the probability for Cage A:
\[
P_A = \binom{7}{3} \times (0.4)^3 \times (0.6)^4 \approx 0.2903.
\]
Step 2: Compute the probability for Cage B:
\[
P_B = \binom{7}{3} \times (0.6)^3 \times (0.4)^4 \approx 0.1935.
\]
Step 3: Compare the probabilities. Since \(P_A > P_B\), the observed sequence is more likely from Cage A.
Final Decision: Cage A.
\end{tcolorbox}


One major finding from these flags is that GPT3.5 uses only the likelihood to make a decision (about 80\% of the time). We can interpret this as applying our structural logit model with zero weight on the prior. This error was also seen in few responses from GPT-4, but this was rare. Exactly one such error was seen in GPT4o. This suggests a rationale for why we found multiple types in the GPT3.5 data, about 80\% are trying to respond using the likelihood alone and 20\% are conceptually Bayesian. This also validates the finding of a single type in GPT4 and GPT4o responses, and confirming that they are mainly noisy Bayesians. The two flags lead to the same conclusion, and are intended to be a check on each other. 


\begin{figure}[h!]
    \centering
    \caption{Average Error Scores by Model (Mean ± SEM) (N=1200)}
    \includegraphics[width=1.0\linewidth]{figs/text2.png}
    
    \label{fig:enter-label}
\end{figure}

\subsubsection{Calculation and Numerical Errors} 

The next three questions (flags 6, 7, 8) tried to capture if the response explicitly computed key numerical values correctly: the prior, the likelihood, and the posterior. This criteria is fairly strict, the response needs to contain the exact value in order to pass. Note that in some cases you do not need to compute an exact value, especially when the true posterior probabilities are near 0 or 1. It is only when the posteriors are very close to 0.5, does the real need for an exact calculation arise. With respect to posterior calculation, we noted that simply computing posterior ratios and comparing them is sufficient for a correct answer. Thus this grading flag permitted the responses to either compute the posterior or get away with simply computing the posterior ratio numerator and denominator. 

\begin{tcolorbox}[breakable, title={GPT4o Omits the Combinatorial Expression}, fontupper=\scriptsize]
First, find the probability of getting this exact outcome from each cage.\medskip

\noindent
Cage A Calculation:\par
Probability = (N balls: $4/10^4$) * (G balls: $6/10^3$)\par
= $(0.4)^4 * (0.6)^3$\par
= 0.01638\medskip

\noindent
Cage B Calculation:\par
Probability = (N balls: $6/10^4$) * (G balls: $4/10^3$)\par
= $(0.6)^4 * (0.4)^3$\par
= 0.02304\medskip

Next, these probabilities are weighted by the chance of using each cage
(\(P(A)=0.7\) vs. \(P(B)=0.3\)):

\[
\text{Final Probability (A)} = 0.7 \times 0.01638 = 0.01147,
\quad
\text{Final Probability (B)} = 0.3 \times 0.02304 = 0.00691.
\]

Because \(0.01147 > 0.00691\), we conclude:\medskip

Final answer: Cage A.
\end{tcolorbox}

The error distributions in figure \ref{fig:calc-error} reveal a few findings. First, since GPT3.5 does not use the prior and typically decides based on the likelihood alone, it never computes the posterior correctly. GPT4 and GPT4o do use the prior in most cases. GPT3.5 and GPT4 struggle with computing the likelihood exactly, while generally GPT4o is able to do so. One common way that GPT3.5 and GPT4 get the likelihood wrong is to omit the combinatorial expression in the formula.  GPT4 and GPT4o almost always uses Bayes Rule to calculate the posterior, but GPT4 makes far more calculational errors than GPT4o.

\begin{figure}[h!]
    \centering
     \caption{Calculation and Numerical Errors by Model (Mean ± SEM) (N=1200)}
    \includegraphics[width=1.0\linewidth]{figs/text3.png}
    \label{fig:calc-error}
\end{figure}

\subsubsection{Last Second Decision Inconsistency}

The last flag tries to get at decision inconsistency or decision noise. Since some GPTs never try to compute the posterior or decide based off the likelihood, it is hard to even define decision noise in some cases. One way to do this is to ask if the model went against the grain of its own overall flow and decision-making rubric right at the last minute and contradicted itself. So if we were to evaluate GPT3.5 we would treat its likelihood calculation as its best guess for the posterior and then check if despite computing a larger value for one cage did it then select the other. If we were evaluating a GPT4 who applies Bayes rule correctly but gets the posterior calculation wrong, we would evaluate inconsistency if its answers against the grain of this incorrect value. 

\begin{tcolorbox}[breakable, title={GPT3.5 Takes a Decision Against Its Calculated Numbers}, fontupper=\small]

\textbf{Step 1:} Compute probabilities for 3 "N" and 3 "G" from each cage.

\medskip
\noindent
\textit{Cage A:} 
Probability of "N" = 4/6 = 2/3, 
Probability of "G" = 2/6 = 1/3.\\
Hence, 
\[
(2/3)^3 \times (1/3)^3 = \frac{8}{729}
\]

\noindent
\textit{Cage B:} 
Probability of "N" = 3/6 = 1/2, 
Probability of "G" = 1/2.\\
Hence,
\[
(1/2)^3 \times (1/2)^3 = \frac{1}{64} 
\]

\medskip
\textbf{Step 2:} The probability of getting 3 "N" balls and 3 "G" balls is higher for Cage A (8/729) compared to Cage B (1/64). Make a decision based on the higher probability outcome.

Final answer: Cage A.

\end{tcolorbox}

One way that such decision errors (typically in GPT4o) happen is that the GPTs correctly compute the posterior but make another final arithmetic error while reducing the fraction or reducing to decimals. This is strictly speaking a numerical error, but since this happens after a correct posterior calculation, the grader picks this up as a decision error. The other way such errors can happens is that after correctly computing the posteriors GPT at the last second overrides itself and reverts to the representativeness  heuristic. Another way this error can happen is that the GPT simply faily to ``interpret" the fraction. This could also be interpreted as an issue or bias rather than decision error. For these reasons these ``inconsistency errors" should be treated as the number of times the GPT made an error after computing the decision metric it was trying to calculate. For these reasons, we advise caution when interpreting this error as ``decision noise". All models do show a few cases of such ``last second errors", but we do not have the power to distinguish between them or the percentage of true ``decision noise". GPT3.5 appears to make more of these errors, suggesting confirmation of the finding of larger decision noise for GPT3.5 in the structural logit model estimates. GPT4o has slightly more such errors than GPT4 because it actually tries to compute the posterior more frequently than GPT4, and in doing so it opens itself to the possibility of making additional algebraic mistakes even when it computes the likelihood correctly. 

\begin{figure}[h!]
    \centering
   \caption{Average Error Scores by Model (Mean ± SEM) (N=1200)} 
    \includegraphics[width=0.5\linewidth]{figs/text4.png}
    
    \label{fig:enter-label}
\end{figure}


\subsubsection{Summary of Analysis of Automated Grading}

The main takeaway from automated grading analysis is that (1) in general, reading and writing errors are rare, (2) GPT3.5 mainly uses the likelihood to decide, and does not incorporate or compute the prior at all (3) GPT4 and GPT4o, are at least conceptually Bayesian, (4) GPT3.5 and GPT4 have a high incidence of numerical errors in the computation of the likelihood and posterior (e.g. omitting the combinatorial expression) and (5) GPT4o is nearly flawless with respect to reading, writing and conceptually applying Bayes rule but even it suffers from numerical errors, (6) decision noise is hard to pin down, but we do find some suggestive evidence for it.

\subsection{Manual Investigation of GPT4o's Errors}

\subsubsection{Data and Methodology}

Our second step in investigating the sources of errors was a manual qualitative analysis of GPT4o's outputs. GPT4o is our leading model and we would want to identify more precisely the kinds of errors it makes using a human grader. Automated grading with flags works well if we want to extract a coarse information grid from a larger sample of textual response, however it is not very good at zooming into the text itself and contextualizing errors. Therefore, we conduct a detailed qualitative analysis focusing on GPT4o's responses from the 6-ball Wisconsin experimental design. We first filter out all correct answers and focus on the remaining incorrect ones (306 out of 3850, about 8\%). Our sample consists of 50 responses from the 306 error responses (16\%). In this subset, temperatures ranged from 0.5 to 0.64 where the accuracy rate is 92\% and comparable to GPT4o's overall accuracy rate. 

\subsubsection{Taxonomy of Errors and Relative Shares}

 Overall, we find that GPT4o almost never gives a wrong response \emph{if} it successfully calculates the posterior. However, the converse is not necessarily true: the model arrives at the correct final answer even when its posterior calculation is incorrect approximately 30\% of the time. One way it achieves this is by using a ``shortcut,'' in which it simply compares ``Likelihood of Cage~A~$\times$~Prior for Cage~A'' with ``Likelihood of Cage~B~$\times$~Prior for Cage~B'' which is another way to implement the optimal Bayesian decision rule.

We observed two main categories of errors. The first type, \emph{mathematical calculation errors}, includes multiplication slips (e.g., computing $3^6$ or $4 \times 16$ incorrectly) and difficulties converting fractions to common denominators. Less frequently, GPT4o discards a multiplication factor or ``forgets'' a previously computed number and replaces it with a hallucinated one. The second type of errors, \emph{calculation interruption}, occurs when the model stops before completing the posterior computation for some stated reason (e.g., ``the complexity of the calculation''). In cases of calculation interruption, about a half (48.14\%) resulted in a wrong cage decision, while the same percentage led to a correct one. This suggests that whenever GPT-4o stops before providing the exact posterior value, it may be making a random guess between Cage A and B.

Other errors also arise, but rarely. First, GPT4o may misapply Bayes' formula by omitting or mishandling the combinatorial aspect of the likelihood (i.e. the binomial term). Second, it may round numbers too early, which affects the final posterior only slightly. Third, the model may compute the posterior as a complex fraction but fail to simplify it. Lastly, in some cases, GPT4o detects a mistake, e.g. posterior exceeding 1 and simply halts rather than attempting to correct itself. This can be seen as a sign of ``laziness'' or unawareness of the need to back-trace and self-correct, or it could that GPT ran out of the time it was allocated for this task.

\begin{table}
  \centering
  \caption{Taxonomy of Errors from  the 16\% sample of GPT4o's  incorrect responses}
  \begin{tabular}{ll}
    \toprule
    \textbf{Error} & \textbf{Description} \\
    \midrule
    A: Calculation Error & General arithmetic/fraction mistakes \\
    \quad A1 & Multiplication errors (e.g., $3^6$ miscalculated) \\
    \quad A2 & Mistakes converting to common denominators \\
    \quad A3 & Dropped factors in products \\
    \quad A4 & Forgetting/replacing evaluated numbers \\
    \midrule
    B: Interruption & Stops mid-process before posterior calculation \\
    C: Bayes Formula & Missing combinations/terms in likelihood \\
    D: Early Rounding & Rounds prematurely but final still correct \\
    E: No Simplification & Leaves posterior as large fraction \\
    F: No Final Answer & Confused, ends without stating a Cage \\
    \bottomrule
  \end{tabular}
    
\end{table}


\subsubsection{Errors in different stages of reasoning}

From the second set of findings, we see that errors do not always occur at the same stage. In a typical response, GPT4o follows these steps:
(1) identify the data (priors, draws) and recognize the need for Bayes' rule,
(2) compute likelihoods for Cage~A and Cage~B,
(3) optionally apply the law of total probability,
(4) optionally compute posteriors for A and B,
(5) render a final decision on Cage~A or Cage~B. 

When a \emph{wrong formula} is used, it typically appears early, whereas arithmetic mistakes (e.g., multiplication or fraction handling) tend to occur in the middle. After the model computes a correct posterior, additional errors are rare. In step 1, where GPT4o must identify that Bayes' rule applies and set up the correct formula, the most common misstep is missing or mixing terms in the likelihood (C). By contrast, in step~2 where GPT must calculating likelihoods for each cage, error type~A is more prevalent, especially multiplication slips (A1) or fraction-handling mistakes (A2). Sometimes, the model forgets factors (A3) or replaces computed values with irrelevant ones (A4). In step 3, when applying the law of total probability and in step~4 where the posterior is calculated, we see more interruption errors (B) and fraction-handling issues (A2, A3, A4). Additionally, at step 4, the model may leave the posterior in an unwieldy fractional form (E). Despite these challenges, step~5 (choosing Cage~A or Cage~B) is often correct; possibly because GPT4o rethinks its final values or defaults to the right cage even if intermediate calculations are incomplete or flawed.

\begin{table}[h!]
  \centering
   \caption{Common Error Types at Each Logical Step in Reasoning}
  \begin{tabular}{p{0.05\textwidth} p{0.25\textwidth} p{0.2\textwidth} p{0.4\textwidth}}
    \toprule
    \textbf{Index} & \textbf{Step Name} & \textbf{Error Codes} & \textbf{Error Descriptions} \\
    \midrule
    1 & Identify Bayes' Rule
      & C
      & Wrong Bayes' formula: missing or mixing terms \\
    2 & Calculate Likelihoods
      & A1
      & Multiplication mistakes \\
    3 & Compute Total Prob
      & B, A2, A3, A4
      & Interruption, Fraction/denominator errors, Dropping factors, Forgetting values \\
    4 & Compute Posterior
      & A4, B, E
      & Forgetting values, Interruption, No simplification \\
    5 & Final Answer
      & None
      & Generally correct or no new errors introduced \\
    \bottomrule
  \end{tabular}
   
\end{table}

\subsubsection{Manually Computed Error Distributions}


To construct error distributions we define five general categories of errors to characterize the ways in which responses from the GPT4o model deviate from correct application of Bayes rule or from an accurate final decision. Category a, data read-in error, involves misreading problem parameters, such as using an incorrect prior or sample size when reading in the data. Category b, incorrect application of (or not using) Bayes rule, involves mistakes in the application of Bayes rule itself, including omission of binomial coefficients or swapping of posterior and likelihood terms. In category c, posterior calculation error, the model attempts to apply Bayes rule but commits numerical or algebraic errors when computing the posterior probability, such as incorrect exponentiation or fraction simplification. Categories  d and e, final decision errors, both focus on the final decisions, in which d is the unconditional error, where the model chooses the wrong cage independent of other errors made in the same response, and e is the conditional error when the model chooses the wrong cage despite computing the posterior correctly.

\begin{table}[htbp]
\centering
\caption{Distribution of Error Types among 50 GPT4o Responses with Incorrect Posteriors}
\label{tab:gpt4o_error_distribution}
\begin{tabular}{lccc}
\hline
Category & Count & Error Type Occurrence & Description \\
\hline
a & 0 & 0\% & Misreading parameters (e.g.\ priors, draws) \\
b & 0 & 0\% & Incorrect or missing Bayes rule setup \\
c & 46 & 92\% & Numerical or algebraic error computing posterior \\
d & 33 & 66\% & Wrong final cage choice overall \\
e & 1 & 2\% & Correct posterior but final cage choice is flipped \\
\hline
\end{tabular}

\end{table}

Table~\ref{tab:gpt4o_error_distribution} presents the distribution of error types among 50 responses with incorrect posteriors from each model, including GPT-3.5, GPT-4, and GPT-4o. A comparative analysis confirms that all models correctly interpret the input data. Notably, GPT-4o exhibits an exceptionally low error rate in the incorrect application of Bayes' rule. The higher error rate of GPT-3.5 compared to GPT-4 in Category B stems from our definition of this category, which includes cases where Bayes' rule is neither explicitly stated nor applied using the likelihood-prior formulation. As corroborated in Section 6.1, GPT-3.5 seldom explicitly states Bayes' rule but instead employs the likelihood-prior approach, reducing the likelihood of identifying such errors. The conditional error in the final decision (Category e) further indicates that more recent models demonstrate improved consistency in their reasoning, making fewer contradictions (``stumbles over" itself less) when deriving final decisions.

\begin{table}[htbp]
\centering
\caption{Error distribution Across 50 ``wrong" response across models}
\label{tab:gpt4o_error_distribution}
\begin{tabular}{lccc}
\hline
Category& GPT3.5 & GPT4 &GPT4o\\
\hline
a & 0\% & 0\% & 0\% \\
b & 6\% & 16\% & 0\% \\
c & 94\% & 98\% & 92\%\\
d & 64\% & 52\% & 66\%\\
e & 22\% & 4\% & 2\%\\
\hline
\end{tabular}

\end{table}


\subsubsection{Examples of GPT4o's Errors}

Below are three examples of GPT-4o's erroneous responses. In the first, GPT4o calculates an incorrect posterior and yet reaches the correct decision. In the second, GPT4o calculates an incorrect posterior and reached the wrong decision. In the third, GPT4o calculates the correct posterior but reached the wrong decision. The exerpts have been trimmed for brevity.  

\begin{figure}[h!]
\centering
\caption{First Example: Incorrect Posterior, Correct Decision}
\label{fig:firstExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\[
P(R\mid A)=15 \times \tfrac{16}{81}\times \tfrac{1}{9}=\tfrac{240}{729},\quad
P(R\mid B)=15 \times \tfrac{1}{16}\times \tfrac{1}{4}=\tfrac{15}{256}.
\]
\textbf{Step 4 (Posterior):}
\[
P(A\mid R)=\frac{P(R\mid A)P(A)}{P(R\mid A)P(A)+P(R\mid B)P(B)}.
\]
\textbf{Claimed Final:} 
\emph{“...the final answer is likely ‘B’ due to Cage B’s higher probability.”}\\
\textit{(Posterior arithmetic is incorrect, but ironically the chosen “B” was the correct cage.)}
\end{tcolorbox}

\end{figure}

\begin{figure}[h!]
\centering
\label{fig:secondExample}
\caption{Second Example: Incorrect Posterior, Wrong Decision}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):}
\[
P(R\mid A)=\tfrac{240}{729},\quad
P(R\mid B)=\tfrac{15}{64}.
\]
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{240}{729}\times0.40}{\dots}\approx 1.208\ (\text{miscomputed}).
\]
\textbf{Final Statement:} 
\emph{“Since we got a probability \textgreater
 1, there's an error. After recalculating, Final: ‘A’.”}\\
\textit{(The correct cage was actually “B,” so the final pick was wrong.)}
\end{tcolorbox}

\end{figure}

\begin{figure}[h!]
\centering
\caption{Third Example: Correct Posterior, Wrong Decision}
\label{fig:thirdExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\[
P(\text{3R,3B}\mid A)=\tfrac{160}{729},\ 
P(\text{3R,3B}\mid B)=\tfrac{5}{16}.
\]
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{160}{729}\times0.60}{\dots},\quad
P(B\mid R)=\frac{\frac{5}{16}\times0.40}{\dots}.
\]
\emph{(Values show $A$ is more likely.)}

\textbf{Final Decision:} \emph{“B”}\\
\textit{(Despite the correct posterior favoring $A$, the model’s final pick was $B$.)}
\end{tcolorbox}

\end{figure}

\subsection{Contrasting Automated and Manual Grading}

We find that automated and manual grading are complementary to each other. The manual grading was not able to detect reading errors or errors where Bayes rule was not applied. That is because these are rare and so the automated grader was able to detect them in a large sample. The manual grading was able to distinguish between (1) calculation mistake and (2) calculation interruption and the relative shares between them, and this was not picked up by the automated grader. Manual grading was also able to pick up one instance of decision noise, and this was also confirmed by the automated grading. Manual grading was also able to pick up finer details about GPT4o that the automated grading could not, but largely the findings from both approaches were similar.  

\subsection{Responses from o1}

Open AI recently released its newest LLM, chatGPT-o1, trained using reinforcement learning methods. According {\it Wikipedia}, ``o1 spends time `thinking' before it answers, making it better at complex reasoning tasks, science and programming than GPT-4o.'' We have not yet performed a full analysis using GPT-o1 subjects, but our initial tests using 36 trials under the Holt-Smith design suggests that GPT-o1 does significantly outperform both human and GPT-4o subjects.
GPT-o1 provided the correct Bayesian posterior in 32 out of 36 trials,  an 89\% accuracy rate that is significantly higher than GPT-4o. GPT-o1 displays greater overall understanding and makes fewer algebraic mistakes.

For example, though GPT-4o typically recognizes the applicability of Bayes Rule and correctly calculates the posterior probability, it frequently fails to realize that the payoff maximizing report in the subsequent ``BDM gamble'' is the Bayesian posterior probability it had already (correctly) calculated. GPT-o1 can also make errors at this stage, but it appears to have the ability to look back and check its own reasoning and self-correct itself when necessary to end up with the correct final answer. 


\begin{figure}[h!]
\caption{Example of a ``self-corrected'' response from GPT-o1}
\label{figure:gpto1}
\begin{blockquote}
\singlespacing

To determine the optimal value of P that maximizes your expected payout, we'll break down the problem step by step.
\medskip

\noindent {\bf Step 1: Determine Posterior Probabilities}
Given the sample  (D,D,D), we update our beliefs about whether the balls were drawn from Urn A or Urn B using Bayes Theorem:

\begin{equation}
P(\text{Urn A} | \text{D,D,D}) = \frac{\frac{1}{27} \times 0.5}{\frac{1}{27} \times 0.5 + \frac{8}{27} \times 0.5} = \frac{1}{9} \approx 0.1111
\end{equation}

\noindent {\bf Step 2: Calculate Expected Payout}
Your expected payout depends on the value of $P$ you choose and the randomly drawn number $U$.
\medskip

\begin{itemize}
\item{Case 1:} $U \le P$. Expected payout: $\frac{1}{9} \times 1000 = 111.11$.
\item{Case 2:} $U > P$. Expected payout: $1000 \times \frac{P + 1}{2} = 500 \times (P + 1)$
\end{itemize}
\medskip

\noindent  Overall expected payout

\begin{equation} E(P) = P \times 111.11 + (1 - P) \times 500 \times \frac{P + 1}{2}.
\label{eq:o1ep}
\end{equation}

\noindent To maximize $E(P)$, take the derivative with respect to $P$ and set it to zero:

\begin{equation}
    \frac{dE}{dP} = -500P + 111.11 = 0.
\end{equation}
\medskip 
\noindent Solving, we get
\begin{equation}
P = \frac{111.11}{500} = 0.2222.
\end{equation}
\medskip
\noindent 
However, upon closer inspection and recalculating, the optimal $ P$ that maximizes the expected payout is: $P=\frac{1}{9} \approx .1111$.

\end{blockquote}
\end{figure}

Figure~\ref{figure:gpto1} shows an example GPT o1 response (slightly edited for brevity) in a trial where it correctly calculated the Bayesian posterior but almost provided a wrong answer due to an algebraic mistake in its calculation of the optimal probability report in the second stage BDM gamble. Specifically, it used an incorrect formula for the expected payoff as a function of its reported probability $P$, $E(P)$ in equation~\ref{eq:o1ep} because it failed to copy the (correct) formula when writing equation~\ref{eq:o1ep}. But at the very end it somehow recognized that it made a mistake, recalculated, and reported the correct posterior probability as its final answer.

\subsection{Conclusion from Analysis of Textual Responses}

While the accuracy and efficiency numbers seem to suggest that GPTs are now on par or better than humans on Bayesian reasoning tasks, a closer look at their textual responses reveals problems that have important implications beyond this narrow experiment. GPTs are quite reliable in reading and writing, as is typically found in copywriting, programming, report writing, legal services, etc. They are also able to correctly apply mathematical concepts, which is useful in the fields of statistical and data analysis and algorithm development. We are also less worried about last minute logical contradictions; they tend to stay on course with their reasoning. However, in domains where exact numerical calculations are critical such as finance, accounting or insurance; GPTs may not yet be sufficiently trustworthy  to replace humans. The problem of ``giving up", ``getting interrupted" or ``laziness" is also an issue here. Textual analysis reveals the \textit{achillies heel} of GPTs which is namely precise, exact and complete numerical computations. 


==> 6_textual_analysis1.tex <==
% analysis of textual responses

Most econometric models treat humans as black-boxes and apart from some research from neuroscience, we do not know exactly how humans process information. However, with GPTs we have the unique advantage of knowing both how their neural ``brains" compute information and the textual response which contains their reasoning behind their answers. Therefore, it makes logical sense to try to parse this text to understand how and why GPTs made mistakes, create a taxonomy of errors and obtain error distributions across models. However, there are some complications. There is more than one way to answer the question correctly and even more ways to make mistakes. The approach we adopted was twofold: (1) create a process for automated grading using a superior GPT model, and (2) manual grading of a smaller sample of GPT4o's responses. 

\subsection{Automated Grading of Textual Responses}

\subsubsection{Data and Methodology}

Due to inherent difficulties in scaling manual grading we came up with a novel algorithm to parse and process GPT's textual responses using a superior GPT model itself. A grading prompt was created which provided the original question, the original answer, the numerical values and logical process that a perfect answer would entail, and detailed instructions on how to mark and grade. After some pilots, we were able to identify 9 yes/no ``flags" that could be raised by a grader GPT in an objective way so as to reduce ambiguity and increase precision. The data consists of a balanced sample of 300 responses per model that were graded by o1 using this grading prompt. We present the error distributions identified by the flags that o1 created. The overall process can be seen in Algorithm~\ref{alg:grading}. 

\begin{algorithm}
\caption{Automated Grading by a Teacher GPT\label{alg:grading}}
\begin{algorithmic}[1]
\State Sample record from data obtaining Original Prompt and Student GPT's Response.
\State Compute an Ideal Answer (teacher's ideal) for each valid prompt-response pair.
\State Build a Grading Prompt combining Original Prompt, Original Response, and Ideal Answer.
\State Send each Grading Prompt to Teacher GPT to obtain a Grading Response.
\State Extract the evaluation flags from Grading Response and store results.
\end{algorithmic}
\end{algorithm}


Table \ref{tab:grading-flags} contains the flags which are categorized into themes. Broadly, we are asking the following questions, (a) did the GPT understand the question and the information present in it? (1-3) (b) did the GPT at least conceptually try to apply Bayes rule? (4-5) (c) did the GPT make numerical errors in calculation? (6-8) (d) did the GPT have any last second logical contradiction in its own reasoning (9)?.

\begin{table}[h!]
\centering
\begin{tabular}{p{1cm} p{4cm} p{9cm}}
\toprule
\textbf{Index} & \textbf{Flag (Yes/No)} & \textbf{Description} \\
\midrule
1 & Cage Composition & Are N vs.\ G compositions used correctly? \\
2 & Draw Count & Are total draws handled correctly? \\
3 & Observed Data & Is the observed outcome properly incorporated? \\
4 & Ignoring Prior & Is the prior probability completely omitted? \\
5 & Conceptual Bayes & Are both prior and likelihood conceptually combined? \\
6 & Prior Computed & Is the prior numerically computed? \\
7 & Likelihood Computed & Is the binomial coefficient applied correctly? \\
8 & Posterior Computed & Are posterior or posterior ratios computed? \\
9 & Inconsistency & Is there a final contradiction in the reported choice? \\
\bottomrule
\end{tabular}
\caption{9-Part Grading Flags from Teacher GPT's Grading Response \label{tab:grading-flags}}
\end{table}

All grading, including human grading, will contain noise, the question is if the noise is below some threshold. A small subset (2.5\%) of the grading was manually evaluated and an error rate of \<2\% was identified. After the grading we looked at the errors identified and manually checked to see if they made sense. There will be some errors that we may not be able to identify due to noise in the grading, but some cannot be explained away as statistical artifacts. This automation, though imperfect, is a scalable way to obtain error distributions and get a sense of what went wrong as the GPT tried to answer the question. We also try to map these flags to try to verify the structural logit model estimates, even though a perfect map is infeasible. 

\subsubsection{Reading and Writing Errors}

The first three questions (Flags 1, 2, and 3) address reading errors, which involve messing up total draws, cage compositions and observed data, as well as writing errors, which involve incorrectly parsing the question’s given data into formulas. We do not expect GPTs to make too many of these errors as one of their strengths is text parsing and text generation. And in line with that expectation we find that most models do not make reading and writing errors, but in rare cases this can happen, even in our leading models. 

\begin{tcolorbox}[breakable, title={GPT3.5 Mixes up the Cage Composition in Step 3}]
\singlespacing
Step 1: Calculate the probability of drawing 4 "N" balls and 3 "G" balls from each cage:
\begin{itemize}
    \item Cage A: \( \left(\frac{4}{10}\right)^4 \times \left(\frac{6}{10}\right)^3 \approx 0.0216 \)
    \item Cage B: \( \left(\frac{6}{10}\right)^4 \times \left(\frac{4}{10}\right)^3 \approx 0.0138 \)
\end{itemize}
Step 2: Compare the probabilities:
\begin{itemize}
    \item The probability for Cage A is higher.
\end{itemize}
Step 3: Note that Cage A has more "N" balls than Cage B.\\[1ex]
Final Decision: Cage A.
\end{tcolorbox}

The full error distribution is presented in Figure \ref{fig:read-write-errors}. The evidence suggests that GPT3.5 makes slightly more such errors than GPT4 or GPT4o and it appears that the one area where the error rate is slightly higher is using information regards the total draws. These types of errors are not part of the structural logit model, which assumes that base information is read correctly. Therefore, the finding that these errors happen very rarely is an indirect validation of the modelling choice of abstracting away from such errors. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/text1.png}
    \caption{Average Reading and Writing Errors by Model (Mean ± SE) (N=1200)}
    \label{fig:read-write-errors}
\end{figure}

\subsubsection{Conceptual and Knowledge Errors}

The next two flags (4 and 5) try to pin down if the response correctly applied Bayes rule, or alternatively made a decision based on the likelihood or priors alone. This question explicitly ignores any numerical considerations and focused squarely on conceptual application. 

\begin{tcolorbox}[breakable, title={GPT4o Decision based on Likelihood Only (Edited for Brevity)}, fontupper=\footnotesize]
Step 1: Compute the probability for Cage A:
\[
P_A = \binom{7}{3} \times (0.4)^3 \times (0.6)^4 \approx 0.2903.
\]
Step 2: Compute the probability for Cage B:
\[
P_B = \binom{7}{3} \times (0.6)^3 \times (0.4)^4 \approx 0.1935.
\]
Step 3: Compare the probabilities. Since \(P_A > P_B\), the observed sequence is more likely from Cage A.
Final Decision: Cage A.
\end{tcolorbox}


One major finding from these flags is that GPT3.5 uses only the likelihood to make a decision (about 80\% of the time). We can interpret this as applying our structural logit model with zero weight on the prior. This error was also seen in few responses from GPT-4, but this was rare. Exactly one such error was seen in GPT4o. This suggests a rationale for why we found multiple types in the GPT3.5 data, about 80\% are trying to respond using the likelihood alone and 20\% are conceptually Bayesian. This also validates the finding of a single type in GPT4 and GPT4o responses, and confirming that they are mainly noisy Bayesians. The two flags lead to the same conclusion, and are intended to be a check on each other. 


\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/text2.png}
    \caption{Average Error Scores by Model (Mean ± SEM) (N=1200)}
    \label{fig:enter-label}
\end{figure}

\subsubsection{Calculation and Numerical Errors} 

The next three questions (flags 6, 7, 8) tried to capture if the response explicitly computed key numerical values correctly: the prior, the likelihood, and the posterior. This criteria is fairly strict, the response needs to contain the exact value in order to pass. Note that in some cases you do not need to compute an exact value, especially when the true posterior probabilities are near 0 or 1. It is only when the posteriors are very close to 0.5, does the real need for an exact calculation arise. With respect to posterior calculation, we noted that simply computing posterior ratios and comparing them is sufficient for a correct answer. Thus this grading flag permitted the responses to either compute the posterior or get away with simply computing the posterior ratio numerator and denominator. 

\begin{tcolorbox}[breakable, title={GPT4o Omits the Combinatorial Expression}, fontupper=\scriptsize]
First, find the probability of getting this exact outcome from each cage.\medskip

\noindent
Cage A Calculation:\par
Probability = (N balls: 4/10^4) * (G balls: 6/10^3)\par
= (0.4)^4 * (0.6)^3\par
= 0.01638\medskip

\noindent
Cage B Calculation:\par
Probability = (N balls: 6/10^4) * (G balls: 4/10^3)\par
= (0.6)^4 * (0.4)^3\par
= 0.02304\medskip

Next, these probabilities are weighted by the chance of using each cage
(\(P(A)=0.7\) vs. \(P(B)=0.3\)):

\[
\text{Final Probability (A)} = 0.7 \times 0.01638 = 0.01147,
\quad
\text{Final Probability (B)} = 0.3 \times 0.02304 = 0.00691.
\]

Because \(0.01147 > 0.00691\), we conclude:\medskip

Final answer: Cage A.
\end{tcolorbox}

The error distributions in figure \ref{fig:calc-error} reveal a few findings. First, GPT3.5 does not explicitly compute the prior confirming the finding that it typically decides using the likelihood alone. GPT4 and GPT4o do compute the prior generally. GPT3.5 and GPT4 struggle with computing the likelihood exactly, while generally GPT4o is able to do so. One common way that GPT3.5 and GPT4 get the likelihood wrong is to omit the combinatorial expression in the formula. GPT3.5 almost never computes the posterior, again because it uses the likelihood. GPT4 and GPT4o do compute the posterior, but GPT4 makes far more calculation errors than GPT4o.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/text3.png}
    \caption{Calculation and Numerical Errors by Model (Mean ± SEM) (N=1200)}
    \label{fig:calc-error}
\end{figure}

\subsubsection{Last Second Decision Inconsistency}

The last flag tries to get at decision inconsistency or decision noise. Since some GPTs never try to compute the posterior or decide based off the likelihood, it is hard to even define decision noise in some cases. One way to do this is to ask if the model went against the grain of its own overall flow and decision-making rubric right at the last minute and contradicted itself. So if we were to evaluate GPT3.5 we would treat its likelihood calculation as its best guess for the posterior and then check if despite computing a larger value for one cage did it then select the other. If we were evaluating a GPT4 who applies Bayes rule correctly but gets the posterior calculation wrong, we would evaluate inconsistency if its answers against the grain of this incorrect value. 

\begin{tcolorbox}[breakable, title={GPT3.5 Takes a Decision Against Its Calculated Numbers}, fontupper=\small]

\textbf{Step 1:} Compute probabilities for 3 "N" and 3 "G" from each cage.

\medskip
\noindent
\textit{Cage A:} 
Probability of "N" = 4/6 = 2/3, 
Probability of "G" = 2/6 = 1/3.\\
Hence, 
\[
(2/3)^3 \times (1/3)^3 = \frac{8}{729}
\]

\noindent
\textit{Cage B:} 
Probability of "N" = 3/6 = 1/2, 
Probability of "G" = 1/2.\\
Hence,
\[
(1/2)^3 \times (1/2)^3 = \frac{1}{64} 
\]

\medskip
\textbf{Step 2:} The probability of getting 3 "N" balls and 3 "G" balls is higher for Cage A (8/729) compared to Cage B (1/64). Make a decision based on the higher probability outcome.

Final answer: Cage A.

\end{tcolorbox}

One way that such decision errors (typically in GPT4o) happen is that the GPTs correctly compute the posterior but make another final arithmetic error while reducing the fraction or reducing to decimals. This is strictly speaking a numerical error, but since this happens after a correct posterior calculation, the grader picks this up as a decision error. The other way such errors can happens is that after correctly computing the posteriors GPT at the last second overrides itself and reverts to the representative heuristic. Another way this error can happen is that the GPT simply faily to ``interpret" the fraction. This could also be interpreted as an issue or bias rather than decision error. For these reasons these ``inconsistency errors" should be treated as the number of times the GPT made an error after computing the decision metric it was trying to calculate. For these reasons, we advise caution when interpreting this error as ``decision noise". All models do show a few cases of such ``last second errors", but we do not have the power to distinguish between them or the percentage of true ``decision noise". GPT3.5 appears to make more of these errors, suggesting confirmation of the finding of larger decision noise for GPT3.5 in the structural logit model estimates. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/text4.png}
    \caption{Average Error Scores by Model (Mean ± SEM) (N=1200)}
    \label{fig:enter-label}
\end{figure}


\subsubsection{Summary of Analysis of Automated Grading}

The main takeaway from automated grading analysis is that (1) in general, reading and writing errors are rare, (2) GPT3.5 mainly uses the likelihood to decide, and does not incorporate or compute the prior at all (3) GPT4 and GPT4o, are at least conceptually Bayesian, (4) GPT3.5 and GPT4 continues to make a lot of numerical errors in computation of the likelihood and posterior (e.g. omitting the combinatorial expression) and (5) GPT4o is nearly flawless with respect to reading, writing and conceptually applying Bayes rule but even it suffers from numerical errors, (6) decision noise is hard to pin down, but we do find some suggestive evidence for it.

\subsection{Manual Investigation of GPT4o's Errors}

\subsubsection{Data and Methodology}

Our second step in investigating the sources of errors was a manual qualitative analysis of GPT4o's outputs. GPT4o is our leading model and we would want to identify exactly what kind of errors does it make. Automated grading with flags works well if we want to extract a coarse information grid from a larger sample of textual response, however it is not very good at zooming into the text itself and contextualizing errors. Therefore, we conduct a detailed qualitative analysis focusing on GPT4o's responses from the 6-ball Wisconsin experimental design. We first filter out all correct answers and focus on the remaining incorrect ones (306 out of 3850, about ~8\%). Our sample consists of 50 responses from this 306 (~16\%). In this subset, temperatures ranged from 0.5 to 0.64 where the accuracy rate is ~92\% and comparable to GPT4o's overall accuracy rate. 

\subsubsection{Types of Errors}

 Overall, we find that GPT4o rarely gives a wrong response \emph{if} it successfully calculates the posterior. However, the converse is not necessarily true: the model sometimes arrives at the correct final answer even when its posterior calculation is incorrect (approximately 30\% of the time). One way it achieves this is by using a ``shortcut,'' in which it simply compares ``Likelihood of Cage~A~$\times$~Prior for Cage~A'' with ``Likelihood of Cage~B~$\times$~Prior for Cage~B.'' This approach is still valid, as it implies an understanding of Bayes' rule.

We observed two main categories of errors. The first type, \emph{mathematical calculation errors}, includes multiplication slips (e.g., computing $3^6$ or $4 \times 16$ incorrectly) and difficulties converting fractions to common denominators. Less frequently, GPT4o discards a multiplication factor or ``forgets'' a previously computed number and replaces it with a hallucinated one. The second type of errors, \emph{calculation interruption}, occurs when the model stops before completing the posterior computation for some stated reason (e.g., ``the complexity of the calculation''). In cases of calculation interruption, about a half (48.14\%) resulted in a wrong cage decision, while the same percentage led to a correct one. This suggests that whenever GPT-4o stops before providing the exact posterior value, it may be making a random guess between A and B.

Other, less significant errors also arise. First, GPT4o may misapply Bayes' formula by omitting or mishandling the combinatorial aspect of the likelihood. Second, it may round numbers too early, which affects the final posterior only slightly. Third, the model may compute the posterior as a complex fraction but fail to simplify it. Lastly, in some cases, GPT4o detects a mistake, e.g. posterior exceeding 1, and simply halts rather than attempting to correct itself. This can see seen as a sign of laziness in back-tracing and self-correcting, or alternatively as a matter of running out of time it allocated for itself for this task.

\begin{table}
  \centering
  \caption{Taxonomy of Errors from Qualitative Analysis of 16\% of GPT4o's Responses that did not match Bayes' Rule.}
  \begin{tabular}{ll}
    \toprule
    \textbf{Error} & \textbf{Description} \\
    \midrule
    A: Calculation Error & General arithmetic/fraction mistakes \\
    \quad A1 & Multiplication errors (e.g., $3^6$ miscalculated) \\
    \quad A2 & Mistakes converting to common denominators \\
    \quad A3 & Dropped factors in products \\
    \quad A4 & Forgetting/replacing evaluated numbers \\
    \midrule
    B: Interruption & Stops mid-process before posterior calculation \\
    C: Bayes Formula & Missing combinations/terms in likelihood \\
    D: Early Rounding & Rounds prematurely but final still correct \\
    E: No Simplification & Leaves posterior as large fraction \\
    F: No Final Answer & Confused, ends without stating a Cage \\
    \bottomrule
  \end{tabular}
\end{table}


\subsubsection{Errors along different Stages of Reasoning}

From the second set of findings, we see that errors do not always occur at the same stage. In a typical response, GPT4o follows these steps:
(1) identify the data (priors, draws) and recognize the need for Bayes' rule,
(2) compute likelihoods for Cage~A and Cage~B,
(3) optionally apply the law of total probability,
(4) optionally compute posteriors for A and B,
(5) render a final decision on Cage~A or Cage~B. 

When a \emph{wrong formula} is used, it typically appears early, whereas arithmetic mistakes (e.g., multiplication or fraction handling) tend to occur in the middle. After the model computes a correct posterior, additional errors are rare. In step 1, where GPT4o must identify that Bayes' rule applies and set up the correct formula, the most common misstep is missing or mixing terms in the likelihood (C). By contrast, in step~2 where GPT must calculating likelihoods for each cage, error type~A is more prevalent, especially multiplication slips (A1) or fraction-handling mistakes (A2). Sometimes, the model forgets factors (A3) or replaces computed values with irrelevant ones (A4). In step 3, when applying the law of total probability and in step~4 where the posterior is calculated, we see more interruption errors (B) and fraction-handling issues (A2, A3, A4). Additionally, at step 4, the model may leave the posterior in an unwieldy fractional form (E). Despite these challenges, step~5 (choosing Cage~A or Cage~B) is often correct; possibly because GPT4o rethinks its final values or defaults to the right cage even if intermediate calculations are incomplete or flawed.

\begin{table}[h!]
  \centering
  \caption{Common Error Types at Each Logical Step in Reasoning}
  \begin{tabular}{p{0.05\textwidth} p{0.25\textwidth} p{0.2\textwidth} p{0.4\textwidth}}
    \toprule
    \textbf{Index} & \textbf{Step Name} & \textbf{Error Codes} & \textbf{Error Descriptions} \\
    \midrule
    1 & Identify Bayes' Rule
      & C
      & Wrong Bayes' formula: missing or mixing terms \\
    2 & Calculate Likelihoods
      & A1
      & Multiplication mistakes \\
    3 & Compute Total Prob
      & B, A2, A3, A4
      & Interruption, Fraction/denominator errors, Dropping factors, Forgetting values \\
    4 & Compute Posterior
      & A4, B, E
      & Forgetting values, Interruption, No simplification \\
    5 & Final Answer
      & None
      & Generally correct or no new errors introduced \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Manually Computed Error Distributions}

To construct error distributions we define five categories of errors to characterize the ways in which responses from the GPT4o model deviate from correct application of Bayes rule or from an accurate final decision. Category 1 involves misreading problem parameters, such as using an incorrect prior or sample size. Category 2 involves mistakes in the application of Bayes rule itself, including omission of binomial coefficients or swapping of posterior and likelihood terms. In category 3, the model attempts to apply Bayes rule but commits numerical or algebraic errors when computing the posterior probability, such as incorrect exponentiation or fraction simplification. Category 4 focuses on the final decision, in which the model may choose the wrong cage because the posterior was never computed correctly. Category 5 is when the model chooses the wrong cage despite computing the posterior correctly but then contradicts it in the final decision.

\begin{table}[htbp]
\centering
\label{tab:gpt4o_error_distribution}
\begin{tabular}{lccc}
\hline
Category & Count & Percentage & Description \\
\hline
1 & 0 & 0\% & Misreading parameters (e.g.\ priors, draws) \\
2 & 0 & 0\% & Incorrect or missing Bayes rule setup \\
3 & 46 & 92\% & Numerical or algebraic error computing posterior \\
4a, unconditional & 35 & 70\% & Wrong final cage choice overall \\
4b, conditional & 1 & 2\% & Correct posterior but final cage choice is flipped \\
\hline
\end{tabular}
\caption{Distribution of Error Types among 50 GPT4o Responses with Incorrect Posteriors}
\end{table}

\subsubsection{Examples of GPT4o's Errors}

Below are three examples of GPT-4o's erroneous responses. In the first, GPT4o calculates an incorrect posterior and yet reaches the correct decision. In the second, GPT4o calculates an incorrect posterior and reached the wrong decision. In the third, GPT4o calculates the correct posterior but reached the wrong decision. The exerpts have been trimmed for brevity.  

\begin{figure}[h!]
\label{fig:firstExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\[
P(R\mid A)=15 \times \tfrac{16}{81}\times \tfrac{1}{9}=\tfrac{240}{729},\quad
P(R\mid B)=15 \times \tfrac{1}{16}\times \tfrac{1}{4}=\tfrac{15}{256}.
\]
\textbf{Step 4 (Posterior):}
\[
P(A\mid R)=\frac{P(R\mid A)P(A)}{P(R\mid A)P(A)+P(R\mid B)P(B)}.
\]
\textbf{Claimed Final:} 
\emph{“...the final answer is likely ‘B’ due to Cage B’s higher probability.”}\\
\textit{(Posterior arithmetic is incorrect, but ironically the chosen “B” was the correct cage.)}
\end{tcolorbox}
\caption{Incorrect Posterior, Correct Decision}
\end{figure}

\begin{figure}[h!]
\label{fig:secondExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):}
\(
P(R\mid A)=\tfrac{240}{729},\quad
P(R\mid B)=\tfrac{15}{64}.
\)
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{240}{729}\times0.40}{\dots}\approx 1.208\ (\text{miscomputed}).
\]
\textbf{Final Statement:} 
\emph{“Since we got a value >1, there's an error. After recalculating, Final: ‘A’.”}\\
\textit{(The correct cage was actually “B,” so the final pick was wrong.)}
\end{tcolorbox}
\caption{Incorrect Posterior, Wrong Decision}
\end{figure}

\begin{figure}[h!]
\label{fig:thirdExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\(
P(\text{3R,3B}\mid A)=\tfrac{160}{729},\ 
P(\text{3R,3B}\mid B)=\tfrac{5}{16}.
\)
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{160}{729}\times0.60}{\dots},\quad
P(B\mid R)=\frac{\frac{5}{16}\times0.40}{\dots}.
\]
\emph{(Values show $A$ is more likely.)}

\textbf{Final Decision:} \emph{“B”}\\
\textit{(Despite the correct posterior favoring $A$, the model’s final pick was $B$.)}
\end{tcolorbox}
\caption{Third Example: Correct Posterior, Wrong Decision}
\end{figure}

\subsection{Contrasting Automated and Manual Grading}

We find that automated and manual grading are complementary to each other. The manual grading was not able to detect reading errors or errors where Bayes rule was not applied. That is because these are rare and so the automated grader was able to detect them in a large sample. The manual grading was able to distinguish between (1) calculation mistake and (2) calculation interruption and the relative shares between them, and this was not picked up by the automated grader. Manual grading was also able to pick up one instance of decision noise, and this was also confirmed by the automated grading. Manual grading was also able to pick up finer details about GPT4o that the automated grading could not, but largely the findings from both approaches were similar.  

\subsection{Responses from o1}

Open AI recently released its newest LLM, chatGPT-o1, trained using reinforcement learning methods. According {\it Wikipedia}, ``o1 spends time `thinking' before it answers, making it better at complex reasoning tasks, science and programming than GPT-4o.'' We have not yet performed a full analysis using GPT-o1 subjects, but our initial tests using 36 trials under the Holt-Smith design suggests that GPT-o1 does significantly outperform both human and GPT-4o subjects.
GPT-o1 provided the correct Bayesian posterior in 32 out of 36 trials,  an 89\% accuracy rate that is significantly higher than GPT-4o. GPT-o1 displays greater overall understanding and makes fewer algebraic mistakes.

For example, though GPT-4o typically recognizes the applicability of Bayes Rule and correctly calculates the posterior probability, it frequently fails to realize that the payoff maximizing report in the subsequent ``BDM gamble'' is the Bayesian posterior probability it had already (correctly) calculated. GPT-o1 can also make errors at this stage, but it appears to have the ability to look back and check its own reasoning and self-correct itself when necessary to end up with the correct final answer. 


\begin{figure}[h!]
\caption{Example of a ``self-corrected'' response from GPT-o1}
\label{figure:gpto1}
\begin{blockquote}
\singlespacing

To determine the optimal value of P that maximizes your expected payout, we'll break down the problem step by step.
\medskip

\noindent {\bf Step 1: Determine Posterior Probabilities}
Given the sample  (D,D,D), we update our beliefs about whether the balls were drawn from Urn A or Urn B using Bayes Theorem:

\begin{equation}
P(\text{Urn A} | \text{D,D,D}) = \frac{\frac{1}{27} \times 0.5}{\frac{1}{27} \times 0.5 + \frac{8}{27} \times 0.5} = \frac{1}{9} \approx 0.1111
\end{equation}

\noindent {\bf Step 2: Calculate Expected Payout}
Your expected payout depends on the value of $P$ you choose and the randomly drawn number $U$.
\medskip

\begin{itemize}
\item{Case 1:} $U \le P$. Expected payout: $\frac{1}{9} \times 1000 = 111.11$.
\item{Case 2:} $U > P$. Expected payout: $1000 \times \frac{P + 1}{2} = 500 \times (P + 1)$
\end{itemize}
\medskip

\noindent  Overall expected payout

\begin{equation} E(P) = P \times 111.11 + (1 - P) \times 500 \times \frac{P + 1}{2}.
\label{eq:o1ep}
\end{equation}

\noindent To maximize $E(P)$, take the derivative with respect to $P$ and set it to zero:

\begin{equation}
    \frac{dE}{dP} = -500P + 111.11 = 0.
\end{equation}
\medskip 
\noindent Solving, we get
\begin{equation}
P = \frac{111.11}{500} = 0.2222.
\end{equation}
\medskip
\noindent 
However, upon closer inspection and recalculating, the optimal $ P$ that maximizes the expected payout is: $P=\frac{1}{9} \approx .1111$.

\end{blockquote}
\end{figure}

Figure~\ref{figure:gpto1} shows an answer  provided by GPT o1 (slightly edited for brevity) to a particular trial where it correctly calculated the Bayesian posterior but almost provided a wrong answer due to an algebraic mistake in its calculation of the optimal probability report in the second stage BDM gamble. Specifically, it used an incorrect formula for the expected payoff as a function of its reported probability $P$, $E(P)$ in equation~\ref{eq:o1ep}, though it did have the correct formula for the conditional expected payoff in the event $U > p$ in Step 2, case 2 just above. Apparently it failed to copy that (correct) formula when writing equation~\ref{eq:o1ep}. But at the very end it appears to have recognized that it made a mistake, recalculated, and reported the correct Bayesian posterior probability as its final answer.

\subsection{Conclusion from Analysis of Textual Responses}

While the accuracy and efficiency numbers seem to suggest that GPTs are now at par or better than humans on Bayesian reasoning tasks, a closer look at their textual responses reveals problems and this has important implications beyond this narrow experiment. GPTs would therefore not face an issue on tasks about reading or writing, as is typically found in copywriting, programming, report writing, legal services, etc. They are also able to correctly apply mathematical concepts, which is useful in the fields of statistical and data analysis and algorithm development. We are also less worried about last minute logical contradictions; they tend to stay on course with their reasoning. However, in domains where exact numerical calculations are essential such as finance, accounting or insurance; GPTs would not be so easily able to replace humans. The problem of ``giving up", ``getting interrupted" or ``laziness" is also an issue here. Textual analysis reveals the \textit{achillies heel} of GPTs which is namely precise, exact and complete numerical computations. 


==> 6_textual_analysis_pranjal.tex <==
% analysis of textual responses

Most econometric models treat humans as black boxes and apart from some research from neuroscience, we do not know exactly how humans process information. However, from the textual responses of GPT, we have the unique advantage of observing the reasoning of GPT subjects, opening the door to analyze where GPTs make mistakes. There are two challenges in such an analysis: the errors made by GPTs can be highly diverse, and the textual responses are not well-structured. We overcome the first challenges by exploiting the simple structure of the binary decision problem, which allows us to classify errors into nine binary error types under four broad categories. To obtain a distribution of GPT errors across categories, we then develop a GPT grader to efficiently process large-scale unstructured responses and determine the value of error types within each category. Key inputs for the GPT grader include an ideal reasoning flow using Bayes' rule and detailed grading rubrics, as well as the original prompt and responses. \ref{appendix:grading_prompts} shows, in detail, the grading prompt. We emphasize that we use a highly capable yet economical model, GPT o3-mini, to grade the three models. The ``teacher" GPT thus grades and evaluates 500 responses per ``student" GPT, demonstrating the scalability of automated grading over human grading. To verify accuracy, we manually reviewed 50 randomly sampled textual responses for each model to verify the o3-mini GPT grader's performance. We also compare the o3-mini grading with grading from GPT o1, the most advanced model, which is costlier to use. Overall, our independent cross-checks confirmed the accuracy of o3-mini's grading and classification of errors in the responses by ChatGPT 3.5, 4 and 4o\footnote{In Appendix \ref{appendix:grader_validation}, we report the fraction of errors in each category from the 50-sample set graded by the human grader, the same 50-sample set by the o1 and o3-mini GPT grader.}.

\subsection{Binary Grading Flags from Textual Responses}

We focus on the textual responses from the 6-ball Wisconsin experiment. The grader is used to generate 9 binary ``grading flags" per response. The first grading flag under Panel A examines whether GPTs understand the context and correctly interpret experimental parameters, including cage composition (i.e., the number of $N$ balls in each cage), sample size ($D$), and the observed number of $N$ balls ($d$). The second grading flag evaluates whether GPT subjects are ``conceptually'' Bayesian by checking if subjects take the prior information into consideration in flag 4 and if they use the sample information as inputs to their decision in flag 5. Flag 4 explicitly checks for representativeness (ignoring the prior) while flag 5 checks for conservatism (ignoring the likelihood). We emphasize the \textit{consideration} of both prior and likelihood in the second category, leaving the examination of \textit{numerically correct} posterior calculation to the third category under Panel C. In Panel C, we check whether the prior probability ($\pi_A$),\footnote{To calculate the prior probability, subjects must understand the process of rolling a 10-sided die and divide the specified range of results for Cage A by 10. While this is straightforward for humans, we occasionally find that GPT subjects use an incorrect numerator or denominator when calculating the prior probability for Cage A. See Appendix  \ref{appendix_error_flag_example} for an example. }  the likelihood probabilities ($f(d|p_A,D)$ and $f(d|p_B,D)$) and the posterior ($\frac{\pi_A f(d|p_A,D)}{\pi_A f(d|p_A,D)+(1-\pi_A) f(d|p_B,D)}$) or posterior odds ($\frac{\pi_A f(d|p_A,D)}{(1-\pi_A) f(d|p_B,D)}$) are correctly calculated. 

There are a few points worth discussing. First, we explicitly instruct the GPT grader to allow for the omission of binomial coefficients when calculating the likelihood, as they will cancel out and do not affect the posterior calculation. Second, we find that some GPT subjects, instead of calculating the posterior probability $\Pi(A|d,\pi,p_A,p_B,D)$ as in equation \ref{eq:bayes_rule}, make decisions by calculating and comparing the product of prior and likelihood, $\pi \times f(d|p_A,D)$ and $(1-\pi) \times f(d|p_B,D)$. This approach is consistent with Bayes' rule, and in such cases, the subject passes flag 8. Third, similar to the identification challenge discussed in \ref{section:identification}, it is sufficient for subjects to make correct decisions if the posterior is on the same side of $1/2$ as the Bayesian posterior. However, since GPT subjects usually report the posterior probabilities, we apply a stricter grading rubric by marking the subject as making an error if their calculated posterior (or posterior odds) was incorrectly calculated even if they provided the correct final answer. 

The final category under Panel D examines whether the final decision (Cage $A$ or $B$) aligns with the previous reasoning, which substantiates the decision noise $\varepsilon$ in the structural logit model. We instruct the GPT grader to read the overall reasoning of the textual responses and then predict the expected outcome based on the reasoning flow. Almost all GPT-4 and 4o subjects answer the problem by calculating the posterior or posterior odds. We define this $\text{flag}=0$ when the final decision contradicts the previous reasoning, such as choosing cage $A$ when the posterior is below $\frac{1}{2}$, or when  $\pi \times f(d|p_A,D)$ is smaller than $(1-\pi) \times f(d|p_B,D)$. In other cases, we ask the GPT grader to explicitly predict the outcome based on the reasoning just before the final answer and compare whether this prediction is consistent with the subjects' report. Note that in this grading flag we \textit{do} penalizing errors in comparing/converting complex fractions right before the final decision.

\subsection{Types of Errors and their Distribution Across Models}

The last three columns in Table \ref{tab:textual_error_distribution} report the percentage of observations for each error\footnote{To demonstrate these granular error types, we provide excerpts from textual responses as example answers classified under each error in Appendix   \ref{appendix_error_flag_example}. }. The link between raw grading flags and error types are as follows. Flags in Panel A, C and D actually detect correct and consistent steps, and so in that case, $\text{error} = 1 - \text{flag}$. In the case of Panel B, the flag detects an error, and so, $\text{error} = \text{flag}$. Panel error rates summarize errors by category. For example, a response is counted as having a Panel A error if it made an error on Flag 1, Flag 2, or Flag 3. The reported percentage is the share of all responses that had at least one error in that specific panel's flags.

The GPT grader evaluates 500 randomly selected text responses for each GPT model, regardless of whether the final decision aligns with Bayes' rule. In the last row, we report the fraction of responses inconsistent with the Bayes' rule. The fraction under all categories doesn't necessarily match the fraction of incorrect responses for two reasons. First, errors are not mutually exclusive. If a subject ignores the prior (error type 4), they will also have errors in calculating the prior (error type 6) and subsequently the posterior (error type 8). Second, since the final decision's consistency with Bayes' rule only requires comparing the posterior to $\frac{1}{2}$, an error in calculating the posterior does not necessarily lead to a mistake in the final decision. 
  
\begin{table}[H]
  \centering
  \caption{Error Distribution from GPT Responses\footnote{Main percentages are based on N=500 responses per model graded by GPT-o3-mini. Numbers in brackets [ ] are results from the human grader on the N=50 validation subset (see Appendix \ref{appendix:grader_validation}) for comparison.}}
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{rlccc}
    \toprule
    \toprule
          & Error Type (Error Rate \%) & GPT 3.5 (\%)  & GPT 4 (\%) & GPT 4o (\%) \\
    \midrule
    \multicolumn{2}{l}{Panel A. Data read-in errors} & 0.4 [2.0] & 0.4 [0.0] & 0.0 [0.0] \\
     \midrule
    1     &  Error reading the compositions of the two cages  & 0.4     & 0.4     & 0.0 \\
    2     &  Error reading the number of balls drawn from  the two cages  & 0.0     & 0.0     & 0.0 \\
    3     &  Error reading the outcome of the draws  & 0.0     & 0.0     & 0.0 \\
     \midrule
    \multicolumn{2}{l}{Panel B. Errors in the application of Bayes Rule} & 82.6 [76.0] & 1.4 [4.0] & 0.6 [0.0]\\
     \midrule
    4     &  Ignoring the prior  & 82.4     & 1.4     & 0.6 \\
    5     &  Ignoring the likelihood  & 0.2    & 0.0     & 0.0 \\
     \midrule
    \multicolumn{2}{l}{Panel C. Errors in computing the posterior probability} & 98.4 [98.0] & 72.0 [82.0] & 21.8 [22.0]\\
     \midrule
    6     &  Error calculating prior probability  & 83.4     & 2.2     & 0.6 \\
    7     &  Error calculating the likelihood  & 70.0     & 67.8     & 13.6 \\
    8     &  Error calculating the posterior (or posterior odds)  & 98.4     & 72.0     & 21.8 \\
     \midrule
    \multicolumn{2}{l}{Panel D. Errors in the final decision} & 4.4 [10.0] & 3.0 [2.0] & 4.6 [14.0]\\
     \midrule
    9     &  Final decision contradicting the previous reasoning & 4.4     & 3.0     & 4.6\\
     \midrule
  \multicolumn{2}{l}{ Fraction of responses inconsistent with Bayes' rule} & 35.2 & 14.2 & 9.2 \\  
 \bottomrule
    \end{tabular}%
  \label{tab:textual_error_distribution}%
  \end{adjustbox}
\end{table}%


Before we dive into the textual analysis, we want to make a caveat that the stated reasoning by the GPT may not fully capture the LLM's complete internal process. That said, table \ref{tab:textual_error_distribution} reinforces our conclusion about the rapid improvement from GPT-3.5 to GPT-4 and GPT-4o, as GPT-4 and GPT-4o make significantly fewer errors in almost all types. This not only reflects higher accuracy, but also indicates fewer mistakes in calculating posterior probabilities or other steps even when final decisions align with Bayes' rule.

Panel A show that that GPT subjects rarely make mistakes in reading experimental parameters (error rates < 0.4\% based on validation checks), suggesting a relatively good understanding of the experimental setup and context. 

Panel B shows a transformation from non-Bayesian to conceptual Bayesian reasoning from GPT-3.5 to GPT-4. A majority of GPT-3.5 decisions rely solely on likelihood, lacking a Bayesian rationality even conceptually let alone numerically (representativeness bias). There is a very tiny fraction of responses where GPT 3.5 ignores the likelihood and makes a decision based on the prior only (conservatism). Our manual review of the text responses shows that they often use representativeness heuristics, making decisions by matching observed patterns in the sample with the composition of the two cages, or simply comparing the likelihood of each cage being the sample's source. Interestingly, GPT-3.5 almost never ignores information in the sample, which indicates that it is more often subject to representativeness rather than conservatism. GPT-4 and GPT-4o almost always demonstrate at least "conceptual Bayesian" reasoning, either by explicitly writing down Bayes' formula or informally considering both prior and likelihood information. 

Panel C highlights another major achievement from ``conceptual Bayesian" to ``perfect Bayesian" when transitioning from GPT-4 to GPT-4o, as the proportion of observations correctly calculating posterior probability rises. This is evident as errors in calculating the posterior probability (error type 8) decrease significantly from ~72\% for GPT-4 to only ~22\% for GPT-4o. We see that GPT-3.5 often does not consider prior information, leading to subsequent errors in prior calculation, while GPT-4 is able to calculate the prior but often struggles with calculating the likelihood. GPT-4o does better, and only struggles a few times with likelihood and posterior calculations. In a majority of the cases, it has essentially solved the underlying mathematical problem. 

Panel D shows that all models are subject to decision noise. Surprisingly, even though GPT-4's overall performance is worse than GPT-4o, its final decision is more consistent with its reasoning process than GPT-4o when comparing the posterior with $\frac{1}{2}$ or comparing the numerator and denominator of posterior odds. To explain this, we first note that GPTs are worse at comparing fractions than rounded decimals. They often attempt to convert fractions to decimals or common denominators for comparison, but may fail when the fractions are too complex. Based on validation samples, GPT-4 more frequently reports posteriors as decimal numbers (43/50 cases), whereas GPT-4o uses fractions more often (17/50 cases). Thus, although GPT-4o calculates the posterior more accurately (often resulting in complex fractions), its greater use of these representations creates more opportunities for errors in the final comparison step. Conversely, GPT-4, while less accurate in initial calculations, uses simpler (though potentially rounded) decimals more often, which are easier to compare correctly relative to its own stated logic. This explains why GPT-4o has a slightly greater error rate under error sub-type 9.\\ 

\begin{figure}[H]
 \centering
 \caption{An example of GPT-4o failing to compare complex fractions}%
 \begin{blockquote}
To determine which cage is more likely to have generated the observed outcome, we use Bayes' theorem to calculate the posterior probabilities. Here's a step-by-step breakdown:\\

 \textbf{Step 1: Determine Posterior Probabilities}
     \[
     P(A \mid \text{3 N and 3 G}) = \frac{P(\text{3 N and 3 G from A}) \times P(A)}{P(\text{3 N and 3 G})}
     \]
     \[
     = \frac{20 \times \frac{8}{729} \times 0.7}{20 \times \frac{8}{729} \times 0.7+20 \times \frac{1}{8}\times 0.3} = \frac{\frac{112}{729}}{\frac{112}{729}+\frac{3}{32}}
     \]
     \[
     = \frac{112}{729} \div \frac{5771}{23328} = \frac{112 \times 23328}{729 \times 5771} = \frac{2612736}{4200459}
     \]

     \[
     P(B \mid \text{3 N and 3 G}) = \frac{P(\text{3 N and 3 G from B}) \times P(B)}{P(\text{3 N and 3 G})}
     \]
     \[
     =\frac{\frac{3}{32}}{\frac{112}{729}+\frac{3}{32}} = \frac{3}{32} \div \frac{5771}{23328} = \frac{3 \times 23328}{32 \times 5771} = \frac{69984}{184672}
     \]\\
 \textbf{Step 2: Make the Decision}\\

Comparing these probabilities, we find that \( P(B \mid \text{3 N and 3 G}) \) is larger than \( P(A \mid \text{3 N and 3 G}) \), suggesting that Cage B is more likely to have generated the observations.

Final answer: Cage B.\\

\textbf{Comments:} Through calculation, we see that \(\frac{2612736}{4200459} = 0.62201202297\), while the true posterior is 0.621036216. With an auto-grader precision of two decimal places, the posterior calculation is considered accurate. However, even though the student obtains the correct posterior in fractional form, they fail in comparing the values.
\end{blockquote}
\end{figure}


\begin{comment}

\subsection{Responses from o1}

Open AI recently released its newest LLM, chatGPT-o1, trained using reinforcement learning methods. According {\it Wikipedia}, ``o1 spends time `thinking' before it answers, making it better at complex reasoning tasks, science and programming than GPT-4o.'' We have not yet performed a full analysis using GPT-o1 subjects, but our initial tests using 36 trials under the Holt-Smith design suggests that GPT-o1 does significantly outperform both human and GPT-4o subjects.
GPT-o1 provided the correct Bayesian posterior in 32 out of 36 trials,  an 89\% accuracy rate that is significantly higher than GPT-4o. GPT-o1 displays greater overall understanding and makes fewer algebraic mistakes.

For example, though GPT-4o typically recognizes the applicability of Bayes Rule and correctly calculates the posterior probability, it frequently fails to realize that the payoff maximizing report in the subsequent ``BDM gamble'' is the Bayesian posterior probability it had already (correctly) calculated. GPT-o1 can also make errors at this stage, but it appears to have the ability to look back and check its own reasoning and self-correct itself when necessary to end up with the correct final answer. 


\begin{figure}[H]
\caption{Example of a ``self-corrected'' response from GPT-o1}
\label{figure:gpto1}
\begin{blockquote}
\singlespacing

To determine the optimal value of P that maximizes your expected payout, we'll break down the problem step by step.
\medskip

\noindent {\bf Step 1: Determine Posterior Probabilities}
Given the sample  (D,D,D), we update our beliefs about whether the balls were drawn from Urn A or Urn B using Bayes Theorem:

\begin{equation}
P(\text{Urn A} | \text{D,D,D}) = \frac{\frac{1}{27} \times 0.5}{\frac{1}{27} \times 0.5 + \frac{8}{27} \times 0.5} = \frac{1}{9} \approx 0.1111
\end{equation}

\noindent {\bf Step 2: Calculate Expected Payout}
Your expected payout depends on the value of $P$ you choose and the randomly drawn number $U$.
\medskip

\begin{itemize}
\item{Case 1:} $U \le P$. Expected payout: $\frac{1}{9} \times 1000 = 111.11$.
\item{Case 2:} $U > P$. Expected payout: $1000 \times \frac{P + 1}{2} = 500 \times (P + 1)$
\end{itemize}
\medskip

\noindent  Overall expected payout

\begin{equation} E(P) = P \times 111.11 + (1 - P) \times 500 \times \frac{P + 1}{2}.
\label{eq:o1ep}
\end{equation}

\noindent To maximize $E(P)$, take the derivative with respect to $P$ and set it to zero:

\begin{equation}
    \frac{dE}{dP} = -500P + 111.11 = 0.
\end{equation}
\medskip 
\noindent Solving, we get
\begin{equation}
P = \frac{111.11}{500} = 0.2222.
\end{equation}
\medskip
\noindent 
However, upon closer inspection and recalculating, the optimal $ P$ that maximizes the expected payout is: $P=\frac{1}{9} \approx .1111$.

\end{blockquote}
\end{figure}

Figure~\ref{figure:gpto1} shows an answer  provided by GPT o1 (slightly edited for brevity) to a particular trial where it correctly calculated the Bayesian posterior but almost provided a wrong answer due to an algebraic mistake in its calculation of the optimal probability report in the second stage BDM gamble. Specifically, it used an incorrect formula for the expected payoff as a function of its reported probability $P$, $E(P)$ in equation~\ref{eq:o1ep}, though it did have the correct formula for the conditional expected payoff in the event $U > p$ in Step 2, case 2 just above. Apparently it failed to copy that (correct) formula when writing equation~\ref{eq:o1ep}. But at the very end it appears to have recognized that it made a mistake, recalculated, and reported the correct Bayesian posterior probability as its final answer.

\end{comment}

\subsection{Conclusion from Analysis of Textual Responses}

We summarize our main finding from the analysis of textual responses here.
\begin{enumerate}
    \item Analyzing the textual responses confirms the rapid improvement from GPT 3.5, to GPT-4 and 4o as more advanced GPTs make less mistakes in almost all error categories.
    \item We observed a remarkable transformation from non-Bayesian to conceptual Bayesian reasoning from GPT-3.5 to GPT-4.
    \item Transitioning from GPT-4 to GPT-4o represents another major leap from ``conceptual Bayesian" to ``perfect Bayesian," achieving the accurate calculation of a Bayesian posterior.
\end{enumerate}

==> 7_conclusion.tex <==
% discussion and conclusion can include a survey of previous literature

Let us return  to the question raised in the title: who is more ``Bayesian''?  Using statistical decision theory, we introduced an objective measure of what it means to be ``more Bayesian'', namely by measuring the subject's {\it decision efficiency,\/} the ratio of the subject's probability of being correct to the optimal probability of being correct implied by Bayes Rule. Our results indicate that while humans generally exhibit high decision efficiency (above 90\%), their performance is heterogeneous and they appear to use a range of heuristics (representativeness, conservatism) in addition to a minority who are best classified as ``noisy Bayesians''. GPT-3.5, meanwhile, is less efficient compared to humans due to calculation errors and ignoring prior information, consistent with the representativeness heuristic. GPT-4’s efficiency is close to human, but these
subjects are not very heterogeneous despite our deliberate attempt to inject heterogeneity via the temperature parameter. GPT-4 subjects are noisy Bayesians due to a significant incidence of calculation errors. GPT-4o nearly eliminates these mistakes, and attains superhuman efficiency in some designs. The latest model o1 is distinctively superhuman. So the answer is that the latest GPT models are more Bayesian than humans. 

Our paper builds on and unites two different strands of the experimental literature: 1) a large literature in economics
and psychology focused on assessing the degree of human rationality in decision-making under uncertainty, 
and 2) a more recent literature that compares the performance of human and AI subjects on a broader range
decision-making tasks and other types of textual and non-textual tasks that require a fair degree of skill,  intelligence, 
and even ``creativity.''

 A growing literature has arisen that directly compares LLMs with humans. The main finding is that LLMs excel at textual tasks. \citet{Hubert2024} show that GPT-4 has  superior creativity and elaboration compared to humans in divergent thinking tasks, producing significantly more original and detailed responses. \citet{Yan2024} and \citet{Taloni2023} find that GPT-4 outperformed humans in ophthalmology exams (82.4\% accuracy vs. 75.7\%) and matched junior translators in quality, excelling in fluency. \citet{Herbold2023} showed that in essay writing, GPT-4 surpassed humans in structure, vocabulary richness, and overall quality. \citet{Martínez2024} found that GPT-4 achieved above-passing performance in the Uniform Bar Examination, placing in the 69th percentile overall. 
 
 However, GPTs often fall short of humans in non-textual tasks requiring reasoning or contextual understanding. \citet{Frieder2023} found that GPT-4 struggled with complex mathematical proofs and computations, performing below expert levels despite surpassing GPT-3.5. \citet{Jones2024} showed that in conversational Turing tests, GPT-4 achieved a 54\% pass rate, lower than humans’ 67\%, and participants were able to identify it based on style. \citet{Li2024} found that in qualitative analysis of healthcare data, GPT-4 missed finer subtleties compared to human researchers. \citet{Yeadon2024} showed that GPT-4 performed lower than university students in physics coding tasks, with outputs often identifiable due to stylistic flaws. \citet{Katz2024} found that despite improvements, GPT-4’s performance on medical board exams fell short of top human physicians in specialties like pediatrics and OB/GYN. 

Our own findings corroborate earlier reports that GPTs are better at textual reasoning rather than mathematical calculations. Our textual error analysis reveals that while early GPTs like GPT3.5 struggled to apply both the right concept, the later GPTs had no issue with recognizing the problem and applying Bayes rule. The issue in the later GPTs continues to be that they struggle with mathematical computations. In our task, they were found to be better than humans at understanding the problem and applying the right concept, but struggled just as much with computation. 

One of our theoretical contributions is to confirm that not only do humans follow  heuristics such as representativeness and conservatism, they also make mistakes. We do not see such issues in GPTs. Therefore, we can trust GPTs to make better decisions under uncertainty than humans, at least more so than the subjects in our sample and on structured tasks where the basic information is available. These results should be interpreted with caution since both human and GPT subjects might behave differently in real-life settings. Additionally, the structural logit framework makes a number of assumptions, monotonicity of response being one of them. It should also be noted that some experiments, e.g. the BDM mechanism, can be additionally confusing to humans, potentially inflating or deflating efficiency estimates.

Future work could test GPTs in dynamic Bayesian updating tasks with real-time feedback. For instance, \citet{Park24} shows that GPT-4 and GPT-4o achieve sublinear regret indicating that they are able to get close to optimal Bayesian updating. Another avenue is studying context specific effects and the effects of taking the task very far away from anything the GPT has observed in its training data. GPTs could also be used to take the place of rational human decision-makers in simulation experiments.  

The main takeaway message from our paper is that humans, compared to AI, rely on heuristics and make more mistakes; they are not as Bayesian as AI. But while the fears of automation are real, humans will continue to play a role because there will always be many more ways of thinking like a human than thinking like a machine. Perhaps, our biases and diverse viewpoints might be the very thing that helps us stay relevant in the age of AI.  




==> backups/temp.tex <==
\subsubsection{Examples}

Below are three examples of GPT-4o's error responses: the first calculated an incorrect posterior but reached the correct decision (0,0,1,0,0); the second calculated an incorrect posterior and reached the wrong decision (0,0,1,1,0); the third calculated the correct posterior but reached the wrong decision (0,0,0,1,1).

\begin{figure}[h!]
\caption{First example of error response from GPT-4o}
\label{figure:GPT-4o}
\begin{blockquote}
\singlespacing
To solve this problem, we need to use Bayes' Theorem to determine which cage is more likely to have been used, given the outcome of 4 red balls and 2 blue balls. We'll break this into steps:

\noindent {\bf{Step 1: Define the Events}}
- Let \( A \) be the event that Cage A was selected.
- Let \( B \) be the event that Cage B was selected.
- Let \( R \) be the event of drawing 4 red balls and 2 blue balls.

\noindent {\bf{Step 2: Determine the Prior Probabilities}}
- \( P(A) = 0.30 \)
- \( P(B) = 0.70 \)

\noindent {\bf{Step 3: Determine the Probability of Drawing 4 Red and 2 Blue Balls from Each Cage}}
For Cage A:
Using the binomial distribution, the probability of drawing 4 red balls and 2 blue balls from Cage A:

\begin{equation} P(R \mid A) = 15 \times \frac{16}{81} \times \frac{1}{9} = \frac{240}{729} \end{equation}

For Cage B:

Using the binomial distribution, the probability of drawing 4 red balls and 2 blue balls from Cage B:

\begin{equation}P(R \mid B) = 15 \times \frac{1}{16} \times \frac{1}{4} = \frac{15}{256}
\end{equation}

\noindent {\bf{Step 4: Use Bayes' Theorem to Calculate the Posterior Probabilities}}

\begin{equation} P(A \mid R) = \frac{P(R \mid A) \cdot P(A)}{P(R \mid A) \cdot P(A) + P(R \mid B) \cdot P(B)} = \frac{\frac{240}{729} \cdot 0.30}{\frac{240}{729} \cdot 0.30 + \frac{15}{256} \cdot 0.70} \end{equation}

\begin{equation} P(B \mid R) = \frac{P(R \mid B) \cdot P(B)}{P(R \mid A) \cdot P(A) + P(R \mid B) \cdot P(B)} = \frac{\frac{15}{256} \cdot 0.70}{\frac{240}{729} \cdot 0.30 + \frac{15}{256} \cdot 0.70} \end{equation}


\noindent {\bf{Step 5: Compare the Posterior Probabilities}}
We compute these probabilities to see which is greater. After simplifying and comparing these values, we decide based on which posterior probability is higher.

\noindent {\bf{Step 6: Final Decision}}
After performing the calculations, if \( P(A \mid R) > P(B \mid R) \), then ""Final Answer: A"". Otherwise, ""Final Answer: B"".

Given the complexity of the fractions and the calculations involved, you would typically perform these calculations using a calculator or computational tool to determine the exact probabilities. Based on this setup, the final answer is likely ""Final Answer: B"" due to the initial higher probability of selecting Cage B and its configuration.
\end{blockquote}
\end{figure}



\begin{figure}[h!]
\caption{Second example of error response from GPT-4o}
\label{figure:gpto1}
\begin{blockquote}
\singlespacing
"To solve this problem, we will use Bayes' theorem to determine the probability that the sample of 6 balls was drawn from Cage A given that the sample contains 4 red balls and 2 blue balls. Let's break down the problem into steps:

### Step 1: Define the Events
- Let \( A \) be the event that the balls are drawn from Cage A.
- Let \( B \) be the event that the balls are drawn from Cage B.
- Let \( R \) be the event that the sample contains 4 red balls and 2 blue balls.

### Step 2: Determine the Probabilities
- The probability that Cage A is selected: \( P(A) = 0.40 \)
- The probability that Cage B is selected: \( P(B) = 0.60 \)

### Step 3: Calculate the Probability of Drawing 4 Red Balls and 2 Blue Balls from Each Cage
- **For Cage A:**
  - Probability of drawing a red ball from Cage A: \( P(\text{red} | A) = \frac{4}{6} = \frac{2}{3} \)
  - Probability of drawing a blue ball from Cage A: \( P(\text{blue} | A) = \frac{2}{6} = \frac{1}{3} \)
  - The probability of drawing exactly 4 red balls and 2 blue balls from Cage A (with replacement) is given by the binomial probability formula:
  \[
  P(R | A) = \binom{6}{4} \left(\frac{2}{3}\right)^4 \left(\frac{1}{3}\right)^2
  \]
  \[
  P(R | A) = 15 \times \left(\frac{16}{81}\right) \times \left(\frac{1}{9}\right) = 15 \times \frac{16}{729} = \frac{240}{729}
  \]

- **For Cage B:**
  - Probability of drawing a red ball from Cage B: \( P(\text{red} | B) = \frac{3}{6} = \frac{1}{2} \)
  - Probability of drawing a blue ball from Cage B: \( P(\text{blue} | B) = \frac{3}{6} = \frac{1}{2} \)
  - The probability of drawing exactly 4 red balls and 2 blue balls from Cage B (with replacement) is given by the binomial probability formula:
  \[
  P(R | B) = \binom{6}{4} \left(\frac{1}{2}\right)^4 \left(\frac{1}{2}\right)^2
  \]
  \[
  P(R | B) = 15 \times \frac{1}{16} \times \frac{1}{4} = 15 \times \frac{1}{64} = \frac{15}{64}
  \]

### Step 4: Apply Bayes' Theorem
We want to find \( P(A | R) \), the probability that the balls were drawn from Cage A given that the sample contains 4 red balls and 2 blue balls. By Bayes' theorem:
\[
P(A | R) = \frac{P(R | A) \cdot P(A)}{P(R)}
\]
where:
\[
P(R) = P(R | A) \cdot P(A) + P(R | B) \cdot P(B)
\]

Calculate \( P(R) \):
\[
P(R) = \frac{240}{729} \times 0.40 + \frac{15}{64} \times 0.60
\]

Convert fractions to a common denominator:
- Convert \(\frac{240}{729}\) to a denominator of 64: \( \frac{240}{729} \approx \frac{240 \times 64}{729 \times 64} \approx \frac{15360}{46656} \)
- Convert \(\frac{15}{64}\) to a denominator of 729: \( \frac{15}{64} \approx \frac{15 \times 729}{64 \times 729} = \frac{10935}{46656} \)

Calculate \( P(R) \):
\[
P(R) = \frac{15360}{46656} \times 0.40 + \frac{10935}{46656} \times 0.60
\]
\[
P(R) = \frac{6144}{46656} + \frac{6561}{46656} = \frac{12705}{46656}
\]

Now calculate \( P(A | R) \):
\[
P(A | R) = \frac{\frac{240}{729} \times 0.40}{\frac{12705}{46656}}
\]
\[
P(A | R) = \frac{\frac{15360}{46656}}{\frac{12705}{46656}}
\]
\[
P(A | R) = \frac{15360}{12705} \approx 1.208
\]

Since \( P(A | R) \) is greater than 1, there must be a calculation error. Let's re-evaluate the problem. The key step is to ensure correct calculation of probabilities and conversion to a common denominator. After recalculating, the correct Bayes' theorem application should lead to a valid probability.

### Final Decision
After recalculating correctly, if \( P(A | R) > P(B | R) \), then the final answer is ""Final Answer: A"", otherwise ""Final Answer: B""."
\end{blockquote}
\end{figure}




\begin{figure}[h!]
\caption{Third example of error response from GPT-4o}
\label{figure:gpto1}
\begin{blockquote}
\singlespacing
"To determine from which cage the sample of 6 balls was likely drawn, given that the sample contains 3 red balls and 3 blue balls, we can use Bayes' Theorem. Here's a step-by-step breakdown of the problem:

### Step 1: Understand the Problem
- There are two cages:
  - **Cage A**: 4 red balls, 2 blue balls.
  - **Cage B**: 3 red balls, 3 blue balls.
- The probability of selecting **Cage A** is 0.60.
- The probability of selecting **Cage B** is 0.40.
- A sample of 6 balls with 3 red and 3 blue balls is drawn.

### Step 2: Define the Probabilities
- Let \( P(A) \) be the probability of selecting Cage A, which is 0.60.
- Let \( P(B) \) be the probability of selecting Cage B, which is 0.40.
- We want to find \( P(A \mid \text{3 red, 3 blue}) \) and \( P(B \mid \text{3 red, 3 blue}) \).

### Step 3: Calculate the Likelihoods
- Calculate the probability of drawing 3 red and 3 blue balls from each cage:

#### For Cage A:
- Probability of drawing a red ball from Cage A: \( \frac{4}{6} = \frac{2}{3} \)
- Probability of drawing a blue ball from Cage A: \( \frac{2}{6} = \frac{1}{3} \)

The probability of drawing 3 red and 3 blue balls from Cage A (with replacement) is given by the binomial distribution:
\[
P(\text{3 red, 3 blue} \mid A) = \binom{6}{3} \left(\frac{2}{3}\right)^3 \left(\frac{1}{3}\right)^3
\]
\[
= 20 \times \frac{8}{27} \times \frac{1}{27} = 20 \times \frac{8}{729} = \frac{160}{729}
\]

#### For Cage B:
- Probability of drawing a red ball from Cage B: \( \frac{3}{6} = \frac{1}{2} \)
- Probability of drawing a blue ball from Cage B: \( \frac{3}{6} = \frac{1}{2} \)

The probability of drawing 3 red and 3 blue balls from Cage B (with replacement) is:
\[
P(\text{3 red, 3 blue} \mid B) = \binom{6}{3} \left(\frac{1}{2}\right)^3 \left(\frac{1}{2}\right)^3
\]
\[
= 20 \times \frac{1}{8} \times \frac{1}{8} = 20 \times \frac{1}{64} = \frac{20}{64} = \frac{5}{16}
\]

### Step 4: Apply Bayes' Theorem
We now use Bayes' Theorem to calculate the posterior probabilities:
\[
P(A \mid \text{3 red, 3 blue}) = \frac{P(\text{3 red, 3 blue} \mid A) \times P(A)}{P(\text{3 red, 3 blue})}
\]
\[
P(B \mid \text{3 red, 3 blue}) = \frac{P(\text{3 red, 3 blue} \mid B) \times P(B)}{P(\text{3 red, 3 blue})}
\]

Where:
\[
P(\text{3 red, 3 blue}) = P(\text{3 red, 3 blue} \mid A) \times P(A) + P(\text{3 red, 3 blue} \mid B) \times P(B)
\]

Calculating the denominator:
\[
P(\text{3 red, 3 blue}) = \frac{160}{729} \times 0.60 + \frac{5}{16} \times 0.40
\]

Convert fractions to a common denominator:
- \(\frac{160}{729} \times 0.60 = \frac{96}{729}\)
- \(\frac{5}{16} \times 0.40 = \frac{2}{16} = \frac{91.125}{729}\)

\[
P(\text{3 red, 3 blue}) = \frac{96}{729} + \frac{91.125}{729} = \frac{187.125}{729}
\]

Now calculate the posterior probabilities:
\[
P(A \mid \text{3 red, 3 blue}) = \frac{\frac{160}{729} \times 0.60}{\frac{187.125}{729}} = \frac{96}{187.125}
\]

\[
P(B \mid \text{3 red, 3 blue}) = \frac{\frac{5}{16} \times 0.40}{\frac{187.125}{729}} = \frac{91.125}{187.125}
\]

### Step 5: Compare the Probabilities
Since the calculations show that the probability of the sample coming from Cage B (\(\frac{91.125}{187.125}\)) is greater than the probability of it coming from Cage A (\(\frac{96}{187.125}\)), the sample is more likely to have come from Cage B.

### Final Decision
Final Answer: B"
\end{blockquote}
\end{figure}



\subsection{Manual Investigation of GPT4o's Errors}

\subsubsection{Data and Methodology}


\subsubsection{Data and Methodology}

Our second step in investigating the sources of errors was a manual qualitative analysis of GPT4o's outputs. GPT4o is our leading model and we would want to identify exactly what kind of errors does it make. We generated 3850 responses from GPT4o, from which the erroneous responses that didn't match the Bayes' Rule is 7.95\%. Then we examined about 16\% of the erroneous responses by random selection. Overall, we find that GPT4o rarely gives a wrong response \emph{if} it successfully calculates the posterior. However, the converse is not necessarily true: the model sometimes arrives at the correct final answer even when its posterior calculation is incorrect (approximately 30\% of the time). One way it achieves this is by using a ``shortcut,'' in which it simply compares ``Likelihood of Cage~A~$\times$~Prior for Cage~A'' with ``Likelihood of Cage~B~$\times$~Prior for Cage~B.'' This approach is still valid, as it implies an understanding of Bayes' rule.

We observed two main categories of errors. The first type, \emph{mathematical calculation errors}, includes multiplication slips (e.g., computing $3^6$ or $4 \times 16$ incorrectly) and difficulties converting fractions to common denominators. Less frequently, GPT4o discards a multiplication factor or ``forgets'' a previously computed number and replaces it with a hallucinated one. The second type of errors, \emph{calculation interruption}, occurs when the model stops before completing the posterior computation for some stated reason (e.g., ``the complexity of the calculation''). In cases of calculation interruption, about a half (48.14\%) resulted in a wrong cage decision, while the same percentage led to a correct one. This suggests that whenever GPT-4o stops before providing the exact posterior value, it may be making a random guess between A and B.

Other, less significant errors also arise. First, GPT4o may misapply Bayes' formula by omitting or mishandling the combinatorial aspect of the likelihood. Second, it may round numbers too early, which affects the final posterior only slightly. Third, the model may compute the posterior as a complex fraction but fail to simplify it. Lastly, in some cases, GPT4o detects a mistake (such as a posterior exceeding 1) and simply halts rather than attempting to correct itself—possibly a sign of laziness in back-tracing and self-correcting, or a matter of running out of time.

\begin{table}
  \centering
  \caption{Taxonomy of Errors from Qualitative Analysis of 16\% of GPT4o's Responses that did not match Bayes' Rule.}
  \begin{tabular}{ll}
    \toprule
    \textbf{Error} & \textbf{Description} \\
    \midrule
    A: Calculation Error & General arithmetic/fraction mistakes \\
    \quad A1 & Multiplication errors (e.g., $3^6$ miscalculated) \\
    \quad A2 & Mistakes converting to common denominators \\
    \quad A3 & Dropped factors in products \\
    \quad A4 & Forgetting/replacing evaluated numbers \\
    \midrule
    B: Interruption & Stops mid-process before posterior calculation \\
    C: Bayes Formula & Missing combinations/terms in likelihood \\
    D: Early Rounding & Rounds prematurely but final still correct \\
    E: No Simplification & Leaves posterior as large fraction \\
    F: No Final Answer & Confused, ends without stating a Cage \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Errors along different Stages of Reasoning}


From the second set of findings, we see that errors do not always occur at the same stage. In a typical response, GPT4o follows these steps:
(1) identify the data (priors, draws) and recognize the need for Bayes' rule,
(2) compute likelihoods for Cage~A and Cage~B,
(3) optionally apply the law of total probability,
(4) optionally compute posteriors for A and B,
(5) render a final decision on Cage~A or Cage~B. 

When a \emph{wrong formula} is used, it typically appears early, whereas arithmetic mistakes (e.g., multiplication or fraction handling) tend to occur in the middle. After the model computes a correct posterior, additional errors become less common.

In step~1, where GPT4o must identify that Bayes' rule applies and set up the correct formula, the most common misstep is error type~C (missing or mixing terms in the likelihood). By contrast, in step~2 (calculating likelihoods for each cage), error type~A is more prevalent, especially A1 (multiplication slips) or A2 (fraction-handling mistakes). Sometimes, the model forgets factors (A3) or replaces computed values with irrelevant ones (A4).

In step~3 (law of total probability) and step~4 (Bayes' posterior calculation), interruption errors (B) and fraction-handling issues (A2, A3, A4) can still crop up. Additionally, at step~4, the model may leave the posterior in an unwieldy fractional form (error~E). Despite these challenges, step~5 (choosing Cage~A or Cage~B) is often correct—possibly because GPT4o compares its final values or defaults to the right cage even if intermediate calculations are incomplete or flawed.

\begin{table}[h!]
  \centering
  \caption{Common Error Types at Each Logical Step in Reasoning}
  \begin{tabular}{p{0.07\textwidth}p{0.3\textwidth}p{0.55\textwidth}}
    \toprule
    \textbf{Index} & \textbf{Step Name} & \textbf{Common Error Types} \\
    \midrule
    1 & Identify Bayes' Rule 
      & C (Wrong Bayes' formula: missing or mixing terms) \\[6pt]
    2 & Calculate Likelihoods
      & A1 (Multiplication mistakes) \\[6pt]
    3 & Compute Total Probability
      & B (Interruption), A2 (Fraction/denominator errors), A3 (Dropping factors), A4 (Forgetting values) \\[6pt]
    4 & Calculate Posterior 
      & A4 (Forgetting values), B (Interruption), E (No simplification) \\[6pt]
    5 & Final Answer
      & Generally correct or no new errors introduced \\
    \bottomrule
  \end{tabular}
\end{table}

\subsubsection{Examples of GPT4o's Errors}

Below are three examples of GPT-4o's error responses: the first calculated an incorrect posterior but reached the correct decision (0,0,1,0,0); the second calculated an incorrect posterior and reached the wrong decision (0,0,1,1,0); the third calculated the correct posterior but reached the wrong decision (0,0,0,1,1). Below are three trimmed excerpts from GPT-4o responses. 

\begin{figure}[h!]
\label{fig:firstExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\[
P(R\mid A)=15 \times \tfrac{16}{81}\times \tfrac{1}{9}=\tfrac{240}{729},\quad
P(R\mid B)=15 \times \tfrac{1}{16}\times \tfrac{1}{4}=\tfrac{15}{256}.
\]
\textbf{Step 4 (Posterior):}
\[
P(A\mid R)=\frac{P(R\mid A)P(A)}{P(R\mid A)P(A)+P(R\mid B)P(B)}.
\]
\textbf{Claimed Final:} 
\emph{“...the final answer is likely ‘B’ due to Cage B’s higher probability.”}\\
\textit{(Posterior arithmetic is incorrect, but ironically the chosen “B” was the correct cage.)}
\end{tcolorbox}
\caption{Incorrect Posterior, Correct Decision}
\end{figure}

\begin{figure}[h!]
\label{fig:secondExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):}
\(
P(R\mid A)=\tfrac{240}{729},\quad
P(R\mid B)=\tfrac{15}{64}.
\)
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{240}{729}\times0.40}{\dots}\approx 1.208\ (\text{miscomputed}).
\]
\textbf{Final Statement:} 
\emph{“Since we got a value >1, there's an error. After recalculating, Final: ‘A’.”}\\
\textit{(The correct cage was actually “B,” so the final pick was wrong.)}
\end{tcolorbox}
\caption{Incorrect Posterior, Wrong Decision}
\end{figure}

\begin{figure}[h!]
\label{fig:thirdExample}
\begin{tcolorbox}[title=\textbf{GPT-4o Excerpt},colframe=black!50,width=\linewidth]
\footnotesize
\textbf{Step 3 (Likelihoods):} 
\(
P(\text{3R,3B}\mid A)=\tfrac{160}{729},\ 
P(\text{3R,3B}\mid B)=\tfrac{5}{16}.
\)
\textbf{Step 4 (Bayes):}
\[
P(A\mid R)=\frac{\frac{160}{729}\times0.60}{\dots},\quad
P(B\mid R)=\frac{\frac{5}{16}\times0.40}{\dots}.
\]
\emph{(Values show $A$ is more likely.)}

\textbf{Final Decision:} \emph{“B”}\\
\textit{(Despite the correct posterior favoring $A$, the model’s final pick was $B$.)}
\end{tcolorbox}
\caption{Third Example: Correct Posterior, Wrong Decision}
\end{figure}



\clearpage

